Structural Re-weighting Improves Graph Domain Adaptation

In many real-world applications, graph-structured data used for training and testing have differences in distribution, such as in high energy physics (HEP) where simulation data used for training may not match real experiments. Graph domain adaptation (GDA) is a method used to address these differences. However, current GDA primarily works by aligning the distributions of node representations output by a single graph neural network encoder shared across the training and testing domains, which may often yield sub-optimal solutions. This work examines different impacts of distribution shifts caused by either graph structure or node attributes and identifies a new type of shift, named conditional structure shift (CSS), which current GDA approaches are provably sub-optimal to deal with. A novel approach, called structural reweighting (StruRW), is proposed to address this issue and is tested on synthetic graphs, four benchmark datasets, and a new application in HEP. StruRW has shown significant performance improvement over the baselines in the settings with large graph structure shifts, and reasonable performance improvement when node attribute shift dominates.

==> 002-related.tex <==

\section{Related Work}
\label{sec:related}

%\pan{Review: Introduce previous GDA methods~\cite{zhang2019dane, wu2020unsupervised, xiao2022domain, zhu2021shift} to some extent to align with the intro but with more details (Emphasize that they work on dense rep. ). To cite non-graph methods, you may say they (graph) build on xxx methods (non-graph). }

Previous GDA methods extend the idea of invariant representation learning from traditional DA with i.i.d. samples through adversarial training in DANN~\cite{ganin2016domain} or some distance-based minimization between source and target distribution~\cite{long2015learning, zellinger2017central, saito2018maximum}. The existing graph methods instead enforce invariant representation on the dense node representations after the GNN Aggregation. DANE~\cite{zhang2019dane} builds on DANN framework by introducing the domain classifier after the GNN embeddings, and UDAGCN~\cite{wu2020unsupervised} further imposes some inter-graph attention mechanism on top of the adversarial training to result in invariant representation regarding final GNN embeddings.  AdaGIn~\cite{xiao2022domain} adopts the graph infomax to encode global structural information together with conditional adversarial networks for invariant node representation. DGDA~\cite{cai2021graph} uses variational graph auto-encoders to recover with disentangled semantic, domain, and random variables. 

%\pan{Review: Some works also have studied GNNs for out-of-distribution (OOD) generalization. Review them: To deal with node classification, information distanglement~\cite{}, representation mixup~\cite{}, data augmentation (also including contrastive learning)~\cite{park2021metropolis,wu2022knowledge}. Works for graph classification can also be categorized as above~\cite{}. Different from GDA methods, these methods do not assume having data from the test (target) domain. So, their overall goal is still to learn invariant representations which cannot handle the conditional shift problem shown in Fig.~\ref{fig:HEPeg}.  }

In addition to GDA works, many Graph out-of-distribution generalization (GOOD) works share similar ideas. For node classification tasks, there are works with invariant representation learning like SR-GNN~\cite{zhu2021shift}, EERM~\cite{wu2022handling}; disentanglement-based models DisenGCN~\cite{ma2019disentangled}, IPGCN~\cite{ liu2020independence}; data augmentation methods  DropEdge~\cite{rong2019dropedge}, MH-Aug~\cite{park2021metropolis}, mixup for graphs~\cite{wang2021mixup}; self-supervised learning based DGI~\cite{veličković2018deep}, GCC~\cite{qiu2020gcc}, KDGA~\cite{wu2022knowledge}and causality-based Gem~\cite{lin2021generative}. Other graph-level classification tasks can also be summarized into the above categories~\cite{hu2019strategies, zhu2021transfer, miao2022interpretable, chenlearning, li2022learning, han2022g, yang2022learning}. However, one difference from GOOD as opposed to GDA is that they assume there is no given target data, so the above methods are not designed for solving the conditional shift problems induced by graph structure as raised in the introduction. 



%, such as using adversarial training~\cite{zhang2019dane, wu2020unsupervised, liao2021information, xiao2022domain}, distribution moment matching~\cite{zhu2021shift}, information distanglement~\cite{}, representation mixup~\cite{}, data augmentation (also including contrastive learning)~\cite{park2021metropolis,wu2022knowledge}, ad training (also include attributes/graph structure adv.).

\iffalse
Distribution shift problem in general (previous techniques in CV \pan{No need to discuss CV. In the paper, you just need at most 1-2 sentences to summarize the works on CV. However, some sentences can be used such as xxx extend xxx (a cv work) to the graph setting by doing xxx }, popular strategies, including distance-based, adversarial-based, …) 
\begin{itemize}
    \item Traditional papers (DAN~\cite{long2015learning}, JAN~\cite{long2017deep}, DANN~\cite{ganin2016domain}, CDAN~\cite{long2018conditional}, MDD~\cite{zhang2019bridging}, MCD~\cite{saito2018maximum}, instance reweighting papers~\cite{huang2006correcting, sugiyama2008direct, kanamori2009least})
    \item Theoretical paper (Ben David)~\cite{ben2010theory}
    \item Include some works from Han on label shifts~\cite{zhao2019learning, tachet2020domain}
    \item \pan{focus on graphs; less on theory and general methdologies in related work; for those theory and methodologies, you may want to cite them when you discuss your theory and approach.}
\end{itemize} 


Graph distribution shift problems \pan{Yes, this may be more discussed, especially those having not been discussed in intro}
\begin{itemize}
    \item Graph OOD tasks: node classification, graph classification \pan{what I suggest is to first categorize graph and node. Then, discuss different formulations: First more on nodes. On graphs, just use a few sentences }
    \begin{itemize}
        \item Node classification: SRGNN~\cite{zhu2021shift} (domain matching in moment, re-weighted), EERM~\cite{wu2022handling} (generate environment, reduce variance), Graph clustering co-training ~\cite{zhu2022shift} \pan{more pages}
        \item Graph classification: GSAT~\cite{miao2022interpretable}, Papers in NeurIPS 2022~\cite{chenlearning, li2022learning, yang2022learning}, G-mixup~\cite{han2022g} DIR~\cite{} (swithch environment)\pan{less pages}
        \item Both: Mixup for graph~\cite{wang2021mixup}
    \end{itemize}
    \item Pre-training: EGO graph~\cite{zhu2021transfer}, Pre-training papers~\cite{hu2019strategies} 
    \item Graph domain adaptation: UDAGCN~\cite{wu2020unsupervised}, DGDA~\cite{cai2021graph} (graph-level, consider domain disentangle, label disentangle, noise reconstruction), Domain adaptive graph infomax~\cite{xiao2022domain} (cross graph, unsupervised, conditional adver), DANE~\cite{zhang2019dane} (IJCAI, adverarial training)
    \item some survey papers: GOOD~\cite{gui2022good}, GraphOOD surveys~\cite{li2022out}
\end{itemize}
\pan{add those references so that I can check and read.}

Differences compared to our formulation: \pan{Typically, we do not need to spend much space on related work to discuss how we are different. In related work, each paragraph focuses on one concept and at the last sentence, we can say how we are different.}
\begin{itemize}
    \item We focus on node classification tasks since we think that node classification tasks and graph classification tasks should be treated differently. \pan{Why node classification and graph classification should be treated differently is not easy to be addressed. But we may argue why previous graph methods can hardly be used in node tasks, e.g., complexity issues. Also, in the intro, we need to have a good reason to say why node level is important. Why DA problem for node is hard (node feature correlation)? }
    Eg. Invariant components across environments are not suitable in this case (EERM and other causally invariant graph classification tasks) \pan{why? I think it is still suitable. The challenge is not here. It is from complexity and correlated features.}
    \item Other node classification tasks define distribution shift in terms of the node embedding after convolution (eg. SRGNN, EERM, clustering co-training) \pan{I believe this point has to be address sufficiently in intro but not here.}\\
    \textit{Argument:}we can first provide some reasons and justifications for the domain alignment after graph convolution
Arguing that this is not optimal if we rely on the shared transformation over the source and target graphs
Manipulating the edge weights over source graphs can be considered as an additional move which suitable in the graph setting and take into account of graph structure  \pan{This should be in intro. }
\end{itemize}

\fi

==> old-001-introduction.tex <==
\section{Introduction}
\label{sec:intro}


Graph neural networks (GNNs) have recently become the de facto tool to learn the representations of graph-structured data~\cite{}. Although they have achieved outstanding performance on benchmarks~\cite{}, they suffer from performance degeneration in many high-stake real-world applications due to their data-distribution shift between the training and test phases~\cite{good or general ood papers,biom,physics}. 

%Many high-stake applications unfortunately suffer from such a problem~\cite{biom,physics}.
One such application that motivates this study is in high energy physics (HEP)~\cite{gnn in gep}, where GNNs are often trained based on simulation data where plenty of labels can be used and are further applied to label-sparse real experiments~\cite{}. However, real experiments have complicated and time-variant environments that may be different from simulation setups. One notable example is the shift of the pile-up (PU) levels in Large Hadron Collider (LHC) experiments~\cite{}. PU level describes the number of collisions around the leading collision of interest, which may shift over time and be away from that used to generate simulation data. Modeling the data via graphs, the connection patterns between the particles in different PU levels will substantially change, as shown in Fig.~\ref{fig:xx}, which induces a big challenge for GNNs to distinguish particles generated from the leading collision (class LC) from the other collisions (class OC) which is a crucial task in HEP data analysis~\cite{}. A similar type of shift also appears in social/biological networks, where the interaction patterns between nodes with different labels may change over time~\cite{} or across different species~\cite{}, as listed in Table~\ref{tab:xx} %Our work targets these distribution-shift problems in node classification tasks. 

The class of techniques to deal with the graph-data-distribution shift is named graph domain adaptation (GDA)~\cite{}. However, current GDA approaches cannot well address the above problem, as they often adopt DA techniques originally proposed to deal with dense embedding features for CV and NLP tasks~\cite{}. Typically, previous works first run GNNs as a black box to encode the structure and node features into dense node representations and then adopt some regularization to impose the representations invariant across the training (source) and test (target) domains~\cite{zhang2019dane, wu2020unsupervised, xiao2022domain,zhu2021shift}. This procedure largely ignores the impact of GNN computation on the distribution shift problem, in particular the impact of interactions between sparse graph structures and node representations. %in GNN computation impacts the distribution shift problem. 

%However, there is an unresolved yet fundamental question: why should one make the final node representation? Any benefits or limitations?
In this work, we are to open the black box and provide insights into two fundamental questions regarding GDA in node classification problems: \emph{First, why should regularization be added to the final node representations? Will regularizing the node representations in intermediate layers further help?} \emph{Second, are invariant representations across domains actually good?} Answering these questions further inspires new GDA algorithms. % based on structural re-weighting. %The key contributions of this work are to provide insights into these questions, which further inspires new GDA algorithms. 
% \begin{itemize}
%     \item[Q1]: Why we want     
% \end{itemize}

First, we can show that with the goal of invariant representation learning, adding regularization to the final node representations is sufficient if the neighborhood aggregation procedure in the GNN is injective. Regulating intermediate node representations may cause information loss due to the data processing inequality~\cite{}. 

Furthermore, we prove that invariant representation learning may be actually sub-optimal in many cases. To see the problem, we take the HEP example in Fig.~\ref{fig:xx} again: In the low PU level, an unlabeled particle that connects to one LC particle with one OC particle may tend to be in class OC, while in the high PU level, a particle with the same neighborhood may be likely in class LC because more OC particles as the neighbors are expected to label the center particle as class OC. Here, the optimal representations even with the same input features should change across domains rather than keep invariant. We formalize this observation as an issue induced by the node-class-conditional distributions of neighborhoods (defined by the graph structure) shift across two domains, which fails previous GDA methods.

To address such a conditional shift problem, we propose a novel GDA algorithm named structural re-weighting (\proj). \proj estimates the edge probabilities between different classes based on pseudo node labels in the target domain, and then uses such estimation to guide bootstrapping  of neighbors in GNN aggregation over the source graphs, which reduces the conditional shift of neighborhoods. 

We have conduct experiments on synthetic graphs, three real-world graph datasets and one HEP dataset to verify our theory and the effectiveness of \proj. We have observed xxx. 





Note that besides GDA approaches, other methods to learn out-of-distribution (OOD) generalizable GNNs~\cite{} also emphasizing 



This is mainly induced by the node-class-conditional distributions of neighborhoods (defined by the graph structure) change across two domains.


Some assume adversarial training~\cite{zhang2019dane, wu2020unsupervised, liao2021information, xiao2022domain}, distribution moment matching~\cite{zhu2021shift}, information distanglement~\cite{}, representation mixup~\cite{}, data augmentation~\cite{park2021metropolis,wu2022knowledge}.


\cite{zhao2019learning}


such as adversarial training~\cite{zhang2019dane, wu2020unsupervised, liao2021information, xiao2022domain}, distribution moment matching~\cite{zhu2021shift}

, such as using adversarial training~\cite{zhang2019dane, wu2020unsupervised, liao2021information, xiao2022domain}, distribution moment matching~\cite{zhu2021shift}, information distanglement~\cite{}, representation mixup~\cite{}, data augmentation (also including contrastive learning)~\cite{}, ad training (also include attributes/graph structure adv.). Some works on graph out-of-distribution generalization may   


apply DA methods or other regularization methods that improve out-of-distribution generalization

They work on dense representations after a GNN encodes the data but largely ignore the effect of the interaction between node attributes and graph structures (typically sparse) during the encoding process. 



largely ignoring the interaction between node attributes (typically dense) and graph structures (typically sparse) induced by GNN computation
the fact that graph-structured data has node attributes (typically dense) and graph structures (typically sparse) as features, let alone the effect of the entanglement of these two types of features induced by GNN computation. Specifically, a common idea in previous works is to first run GNNs to encode   

whose distribution shifts should be addressed  

DA has been widely applied to CV and NLP tasks~\cite{} and has recently got extended to graph DA (GDA), i.e., solving graph learning tasks~\cite{}.

in node classification      

which trains GNNs by leveraging labels from the training (source) domain and the difference between the graph features between the training and test (target) domains. 



%may have different latent 

Poor quality of inference given by GNNs may mislead scientists and cost    

One of such applications which motivates this study is high energy physics, where GNNs are often trained based on the simulation data whose labels are plenty and further applied to real experiments that are lack of labels~\cite{}. However,      

%(i.e. PS(G, Y ) ̸= PT(G, Y ))



Many applications call for “transferring” graph representations learned from one distribution (domain)
to another, which we refer it as graph domain adaptation (GDA), for instance, temporally
evolved social networks (Wang et al., 2021), molecules of different scaffolds (Hu et al., 2019), and
protein-protein interaction networks in various species (Cho et al., 2016). In general, this setting
of transfer learning is challenging due to the data-distribution shift between the training (source)
and test (target) domains (i.e. PS(G, Y ) ̸= PT(G, Y )). In particular, such a challenge escalates for
graph-structured data that are abstractions of diverse nature

Graph representation learning has been at the center of various real-world applications, such as
drug discovery (Duvenaud et al., 2015), recommender systems (Ying et al., 2018; Sankar et al.,
2021), forecasting (Tang et al., 2020; Derrow-Pinion et al., 2021) and outlier detection (Zhao et al.,
2021a; Deng & Hooi, 2021). In recent years, there has been a surge of interest in developing graph
neural networks (GNNs) as powerful tools for graph representation learning (Kipf &Welling, 2016a;
Veliˇckovi´c et al., 2018; Hamilton et al., 2017; Wu et al., 2019). Remarkably, GNNs have achieved
state-of-the-art performance on numerous graph-related tasks including node classification, graph
classification and link prediction (Chien et al., 2021; You et al., 2021; Kipf & Welling, 2016b).

\begin{itemize}
    \item  General motivations over distribution shift problems (may separate them into OOD generalization, pre-training, domain adaptation, semi-supervised learning tasks, …)  \pan{No need to be so general; Better specified to graph/geometric data; Emphasize potential connection to your scientific application (setting up the words to put readers into a context that is good for you is crucial, e.g., domain adaption + node classification instead of other settings, ); The first paragraph better focuses on the problems instead of the categorization of approaches.}
    \item Some existing works with traditional domains, (CV, NLP, …) \pan{No need to extensively review CV/NLP; Directly say many current graph methods borrow many things from CV/NLP, such as... Here, think about method categorization: pretraining, OOD, (for other methods, do not need to discuss extensively, you may put them into related work)... We focus on domain adaption and why. Do we also want to discuss OOD extensively here?}
    \item GNN applications and the common sense that GNN cannot perform well under distribution shift. Specifically, node classification tasks \pan{It is better to start to argue against what methods have been adopted. What kind of problems do they have? (1) Whether applied to node level? (2) Whether consider graph structure shift? (3)Whether there is a principled solution (theory)? (4) whether graph level solution can be applied to node level tasks? what are the fundamental challenges of DA in node level tasks? (a) the entanglement of node feature shifts and structural shifts, (b) non-iid issues } 
    \item Briefly mention some works in terms of the GNN distribution shift problems \pan{Remove}
    \item List our contributions \pan{We need to first use language to describe how we address the above problems in a logic way before summarizing them into bullets.  }
    \pan{It seems that we miss mentioning the key insights here and the key questions we are to answer: Some key words, node features (distribution) shift, structural (distribution) shift, the pros (information processing inequality) and cons (bootstraping/reweighting) of distribution shift removal after message passing? Our reweighting method can also be applied to aligned with methods that do not rely on shift removal such as mix-up.}
    \begin{itemize}
        \item Formulate the distribution shift/domain adaptation on node classification \pan{(the description here sounds vague; ``Formulate'' does not sound like a contribution)}
        \item Review and fill in the theoretical gap over other related OOD algorithms and DA methods \pan{(the description here sounds vague; what gap? Are we going to review? Are we going to discuss OOD?)}
        \item Argue the insufficiency over previous work and motivate the design of our framework \pan{Argue insufficiency is not a contribution. Are these listed just as a logic flow?} \pan{It seems that we have so many bullets here on the drawback of previous works. We also miss the key insights into our work.}
        \item Synthetic and real experiments (provide another physics dataset)
    \end{itemize}
\end{itemize}

==> old-002-related.tex <==

\section{Related Work}
\label{sec:related}

%\pan{Review: Introduce previous GDA methods~\cite{zhang2019dane, wu2020unsupervised, xiao2022domain, zhu2021shift} to some extent to align with the intro but with more details (Emphasize that they work on dense rep. ). To cite non-graph methods, you may say they (graph) build on xxx methods (non-graph). }

Previous GDA methods extend the idea of invariant representation learning from traditional DA with i.i.d. samples through adversarial training in DANN~\cite{ganin2016domain} or some distance-based minimization between source and target distribution~\cite{long2015learning, zellinger2017central, saito2018maximum}. The existing graph methods instead enforce invariant representation on the dense node representations after the GNN Aggregation. DANE~\cite{zhang2019dane} builds on DANN framework by introducing the domain classifier after the GNN embeddings, and UDAGCN~\cite{wu2020unsupervised} further imposes some inter-graph attention mechanism on top of the adversarial training to result in invariant representation regarding final GNN embeddings.  AdaGIn~\cite{xiao2022domain} adopts the graph infomax to encode global structural information together with conditional adversarial networks for invariant node representation. DGDA~\cite{cai2021graph} uses variational graph auto-encoders to recover with disentangled semantic, domain, and random variables. 

%\pan{Review: Some works also have studied GNNs for out-of-distribution (OOD) generalization. Review them: To deal with node classification, information distanglement~\cite{}, representation mixup~\cite{}, data augmentation (also including contrastive learning)~\cite{park2021metropolis,wu2022knowledge}. Works for graph classification can also be categorized as above~\cite{}. Different from GDA methods, these methods do not assume having data from the test (target) domain. So, their overall goal is still to learn invariant representations which cannot handle the conditional shift problem shown in Fig.~\ref{fig:HEPeg}.  }

In addition to GDA works, many Graph out-of-distribution generalization (GOOD) works share similar ideas. For node classification tasks, there are works with invariant representation learning like SR-GNN~\cite{zhu2021shift}, EERM~\cite{wu2022handling}; disentanglement-based models DisenGCN~\cite{ma2019disentangled}, IPGCN~\cite{ liu2020independence}; data augmentation methods  DropEdge~\cite{rong2019dropedge}, MH-Aug~\cite{park2021metropolis}, mixup for graphs~\cite{wang2021mixup}; self-supervised learning based DGI~\cite{veličković2018deep}, GCC~\cite{qiu2020gcc}, KDGA~\cite{wu2022knowledge}and causality-based Gem~\cite{lin2021generative}. Other graph-level classification tasks can also be summarized into the above categories~\cite{hu2019strategies, zhu2021transfer, miao2022interpretable, chenlearning, li2022learning, han2022g, yang2022learning}. However, one difference from GOOD as opposed to GDA is that they assume there is no given target data, so the above methods are not designed for solving the conditional shift problems induced by graph structure as raised in the introduction. 



%, such as using adversarial training~\cite{zhang2019dane, wu2020unsupervised, liao2021information, xiao2022domain}, distribution moment matching~\cite{zhu2021shift}, information distanglement~\cite{}, representation mixup~\cite{}, data augmentation (also including contrastive learning)~\cite{park2021metropolis,wu2022knowledge}, ad training (also include attributes/graph structure adv.).

\iffalse
Distribution shift problem in general (previous techniques in CV \pan{No need to discuss CV. In the paper, you just need at most 1-2 sentences to summarize the works on CV. However, some sentences can be used such as xxx extend xxx (a cv work) to the graph setting by doing xxx }, popular strategies, including distance-based, adversarial-based, …) 
\begin{itemize}
    \item Traditional papers (DAN~\cite{long2015learning}, JAN~\cite{long2017deep}, DANN~\cite{ganin2016domain}, CDAN~\cite{long2018conditional}, MDD~\cite{zhang2019bridging}, MCD~\cite{saito2018maximum}, instance reweighting papers~\cite{huang2006correcting, sugiyama2008direct, kanamori2009least})
    \item Theoretical paper (Ben David)~\cite{ben2010theory}
    \item Include some works from Han on label shifts~\cite{zhao2019learning, tachet2020domain}
    \item \pan{focus on graphs; less on theory and general methdologies in related work; for those theory and methodologies, you may want to cite them when you discuss your theory and approach.}
\end{itemize} 


Graph distribution shift problems \pan{Yes, this may be more discussed, especially those having not been discussed in intro}
\begin{itemize}
    \item Graph OOD tasks: node classification, graph classification \pan{what I suggest is to first categorize graph and node. Then, discuss different formulations: First more on nodes. On graphs, just use a few sentences }
    \begin{itemize}
        \item Node classification: SRGNN~\cite{zhu2021shift} (domain matching in moment, re-weighted), EERM~\cite{wu2022handling} (generate environment, reduce variance), Graph clustering co-training ~\cite{zhu2022shift} \pan{more pages}
        \item Graph classification: GSAT~\cite{miao2022interpretable}, Papers in NeurIPS 2022~\cite{chenlearning, li2022learning, yang2022learning}, G-mixup~\cite{han2022g} DIR~\cite{} (swithch environment)\pan{less pages}
        \item Both: Mixup for graph~\cite{wang2021mixup}
    \end{itemize}
    \item Pre-training: EGO graph~\cite{zhu2021transfer}, Pre-training papers~\cite{hu2019strategies} 
    \item Graph domain adaptation: UDAGCN~\cite{wu2020unsupervised}, DGDA~\cite{cai2021graph} (graph-level, consider domain disentangle, label disentangle, noise reconstruction), Domain adaptive graph infomax~\cite{xiao2022domain} (cross graph, unsupervised, conditional adver), DANE~\cite{zhang2019dane} (IJCAI, adverarial training)
    \item some survey papers: GOOD~\cite{gui2022good}, GraphOOD surveys~\cite{li2022out}
\end{itemize}
\pan{add those references so that I can check and read.}

Differences compared to our formulation: \pan{Typically, we do not need to spend much space on related work to discuss how we are different. In related work, each paragraph focuses on one concept and at the last sentence, we can say how we are different.}
\begin{itemize}
    \item We focus on node classification tasks since we think that node classification tasks and graph classification tasks should be treated differently. \pan{Why node classification and graph classification should be treated differently is not easy to be addressed. But we may argue why previous graph methods can hardly be used in node tasks, e.g., complexity issues. Also, in the intro, we need to have a good reason to say why node level is important. Why DA problem for node is hard (node feature correlation)? }
    Eg. Invariant components across environments are not suitable in this case (EERM and other causally invariant graph classification tasks) \pan{why? I think it is still suitable. The challenge is not here. It is from complexity and correlated features.}
    \item Other node classification tasks define distribution shift in terms of the node embedding after convolution (eg. SRGNN, EERM, clustering co-training) \pan{I believe this point has to be address sufficiently in intro but not here.}\\
    \textit{Argument:}we can first provide some reasons and justifications for the domain alignment after graph convolution
Arguing that this is not optimal if we rely on the shared transformation over the source and target graphs
Manipulating the edge weights over source graphs can be considered as an additional move which suitable in the graph setting and take into account of graph structure  \pan{This should be in intro. }
\end{itemize}

\fi

==> old-003-prelim.tex <==
\section{Preliminaries}  
\label{sec:prelim}

%\pan{General concept of distribution shifts, domain adaption problems, how previous non-graph methods do domain adaptation (previous theoretical results are actually optional, their usage is to lead to previous concept to do (distribution) shift removal). Define graphs; Introduce GNN. say about previous graph DA (always adopt post-MP shift removal).  Others should be put into next section. }

\textbf{Unsupervised Domain Adaptation.}
%\sk{notation in this section need to revise}
Under the unsupervised domain adaptation (UDA) setting, the model has access to labeled data $\{x_i, y_i\}$ from the source domain, and unlabeled data $\{x_i\}$ from the target domain. Denote $\mathcal{P}_S$ and $\mathcal{P}_T$ as the distribution for input $x$ for the source and target domain respectively. Denote $f$ to be the true labeling function that maps inputs to labels and $g$ be the hypothesis function that predicts the labels. The error of hypothesis function $g$ for a domain $U$ is defined as $\epsilon_U(g) = \epsilon_U(g, f_U) = \mathbb{E}_{x\in \mathbb{P}_U}[|g(x)-f_U(x)|]$. The overall objective is to train on source labeled data and test on the unlabeled target data with a small classification error $\epsilon_T(g)$.

In practice, let $\mathcal{Z}$ be a latent space and $\phi$ be the feature transformation function from input space to latent space.  Now, the hypothesis function $g$ is operated on latent space $\mathcal{Z}$ and the function composition $g\circ \phi = g(\phi(\cdot))$ will map an input to its latent representation and then predict the label. Namely, we are aiming to find the $\phi$ and $g$ that achieves the lowest $\epsilon_T(\phi, g, f_T) = \mathbb{E}_{x\in \mathbb{P}_T}[|g(\phi(x))-f_T(x)|]$ through training on the source domain.

Inspired by some generalization bound analysis like~\cite{wu2019domain, ben2010theory}, people formulate some training objectives for DA problems. For instance, as demonstrated below: 
\begin{equation}
\label{bound}
    \begin{aligned}
        \epsilon_{T}(\phi, g) = &\epsilon_{S}(\phi, g) 
        + \int_{z} d\mathcal{P}_T^{\phi}(z) (r_T(z;\phi,g)-r_S(z;\phi,g))\\
        &\quad + \int_{z} (d\mathcal{P}_T^{\phi}(z) - d\mathcal{P}_S^{\phi}(z)) r_S(z;\phi,g)  
    \end{aligned}
\end{equation}
where $d\mathcal{P}_U^{\phi}(z) = \int_{x:\phi(x)=z} d\mathcal{P}_U(x)$ and $r_{U}(z;\phi,g) = \int_{x:\phi(x) = z}|g(z) - f_U(x)|d\mathcal{P}_U(x)$.

The minimization of target error can be decomposed into the minimization of three terms in Eq.~\eqref{bound}. The first term implies the minimization of source error. The second term will become zero if the labeling function is the same for the source and target domains. However, it is not directly controllable without the information of $f(x)$. The third term is will become zero when $\mathcal{P}_S^\phi$ is the same as $\mathcal{P}_T^\phi$. Therefore, combining the minimization goal from the first term and the third term, the optimal model appears to learn domain invariant latent representations with $\mathcal{P}_S^\phi = \mathcal{P}_T^\phi$ which achieves the lowest classification error at the same time. Practically, distance-based algorithms~\cite{} minimize some distance measures like Maximum Mean Discrepancy(MMD) between the source and target latent representations and adversarial-based frameworks~\cite{} aims to find the domain-invariant representations through the adversarial training with domain discriminator.

\textbf{Conditional Shift.} \pan{Review: Some works have studied conditional shift while not for graph-structured data~\cite{zhang2013domain, zhao2019learning,tachet2020domain} (and I think there are more works). Summarize the key ideas of the group of these works. However, these methods all assume that samples are independent and cannot deal with the graph connections between samples. }

\textbf{Graph.}
Let $G=(V,E,X)$ denote a graph with nodes $V$, edges $E$ and nodes are associated with node feature vectors $X_v$ for $v\in V$. For node classification tasks, each node $v \in V$ has a label $y_v$.


\noindent\textbf{Graph Neural Networks.}
GNNs utilize the graph structure and node features to learn node representations $\{H_v, v\in V\}$ for downstream node classification tasks. At each layer of GNN, for each node $v$, GNN aggregates this node's neighborhood information and updates its node representation. After $K$ iterations of neighborhood aggregation, GNN will output final node representations which capture the structure and feature information within the $K$-hop neighborhood. For each iteration: 
\begin{equation}
\resizebox{1\hsize}{!}
    {H_v^{(k)}=\text{UPDATE}\,(H_v^{(k-1)}, \text{AGG}\,(\{H_u^{(k-1)}:u \in N(v)\})), \;H_v^{(0)} = X_v}
    \label{eq:GNN}
\end{equation}
 where $H_v^{(k)}$ stands for the feature vector of node $v$ at $k$-th iteration and $N(v)$ is the set of nodes adjacent to node $v$. This equation can be considered as a generic Message Passing (MP) step, where the AGG function aggregates messages from adjacent nodes and the UPDATE function learns the node representation taking in the aggregated message and its representation from the previous layer.  For node classification tasks, the final obtained node representations $\{H_v^{(K)}, v\in V\}$ are used for predictions.

\textbf{Graph Unsupervised Domain Adaptation. }
Under node classification tasks, we are given the source graph $G_s = (V_S, E_S, X_S)$ with node labels $Y_s$ and unlabeled target graph $G_t = (V_T, E_T, X_T)$. Similarly, the concept of finding a model that balances 1). classification error in source and 2). getting the domain-invariant representations has been adopted by some existing works to the graph setting~\cite{}. Specifically, these models choose to learn the domain invariant node representations after the MP step on graphs. We call this type of algorithm post-MP domain-invariant representation learning. In detail, the algorithm first performs message passing starting from original node features $X_v$ in graphs and obtains node embeddings $H_v$ following the logic in Eq.~\eqref{eq:GNN}. Then, a transformation function $\phi_{post}:\mathcal{H} \rightarrow \mathcal{Z}$ will map the node embeddings after pure MP $H_v$ to domain-invariant latent representation $Z_v$, where $\mathcal{P}_{\mathcal{Z}_S}^{\phi_{post}} = \mathcal{P}_{\mathcal{Z}_T}^{\phi_{post}}$. Sometimes, the transformation function $\phi_{post}$ is embedded as the parameters in GNN during the MP step. \sk{need to polish and add details}

Even though many existing works use the idea of Post-MP invariant representation learning, few analysis has been provided upon this approach. In the next section, we will discuss the benefits and limitations of Post-MP invariant representation learning. 





==> old-004-method-i-113.tex <==
\section{Analysis for Invariant Node Representations}\label{sec:analysis}
% \pan{First give the definition of structural shift and node shift. If we do not have S-shift, when we remove shift in node features. We are always good. If we have structural shift, Intuitively, post-MP shift removal can.... However, the first question is whether shift removal could be added to non-last layer.} 

% \pan{Any benefits for pre-MP shift removal? As long as the MP satisfies injective mapping, adding one pre-MP shift removal is useless. To explain this, we want to use the notation of Eq.~\eqref{eq:GNN}. Just consider one layer. Give the theorem based on information processing inequality. Note here you probably need KL. Also, I did not clearly see whether you need label shift = 0.}

% \pan{Any limitations for just post-MP shift removal? What is the upper bound?}

In this section, we will first analyze and provide the reason why only making the last-layer node representations invariant across domains is optimal, if learning invariant representations is set as the goal (Sec.~\ref{subsec:benefits}). Then, we show that learning invariant representations is actually sub-optimal when the distributions of neighbors conditional on the node label shift across domains (Sec.~\ref{subsec:limitation}). 

\subsection{Optimality of Domain-Invariance in the Last Layer}
\label{subsec:benefits}
As both node attributes and graph structure provide information for making predictions on the graph, the distribution of either of them may shift between domains, named attribute shift and structure shift, respectively,  
which will be formally defined later. Comprehensive analysis should consider three scenarios (a) with only attribute shift, (b) with only structure shift, (c) with attribute + structure shifts. However, as structure shift can be transformed into a distribution shift of node representations (similar to attribute shift) after one-layer MP, we ignore case (b) by always assuming the existence of attribute shift. So, our following discussion only breaks into two cases with or without structure shift. First, we define structure shift and attribute shift.

\textbf{Structure shift.} A naive way to define structure shift is to compare the distributions of adjacent matrices $\bP^{\dS}_{\mA}$ and $\bP^{\dT}_{\mA}$ from two domains respectively. However, this does not consider the effect of node labels. So, we consider the joint distribution with node labels $\bP_{\mA\times \mY}$. As nodes are not ordered, we have $\bP_{\mA\times \mY}(\mA, \my) = \bP_{\mA\times \mY}(\mPi\mA\mPi^\top, \mPi\my)$ for any  $\mPi$. \underline{Structure shift} refers to $\bP_{\mA\times \mY}^\dS\neq\bP_{\mA\times \mY}^\dT$. %Note that this means either label shift $\bP_{\mY}^\dS \neq\bP_{\mY}^\dT$ or label-conditional structure shift. $\bP_{\mA|\mY}^\dS\neq\bP_{\mA|\mY}^\dT$.

\textbf{Attribute shift.} We assume that by not considering the graph structure, the attributes $x_v$, $v\in\dV$ are IID sampled from $\bP_{X|Y}$ given their labels $y_v$. Therefore, the conditional distribution of $\mx|\my$ satisfies $\bP_{\mX|\mY}(\mx|\my) =\prod_{v\in \dV} \bP_{X|Y}(x_v|y_v)$, which satisfies $\bP_{\mX|\mY}(\mx|\my)= \bP_{\mX|\mY}(\mPi\mx|\my)$ for any $\mPi$ such that $\mPi\my=\my$. \underline{Attribute shift} refers to $\bP^\dS_{X|Y}\neq \bP^\dT_{X|Y}$. 

We use the joint distribution to define structure shift while the conditional distribution to define attribute shift because it better aligns with practice: Graph structure models the correlation between nodes including their labels while node attributes are often independent given their labels. 

Our analysis is motivated by the error bound in Eq.~\eqref{eq:bound}. We view the  GNN as $\phi$ to transform the node attributes and the graph structure into node representations $\mh^{(L)}=\phi(\mx,\mA)$ and the downstream node classifier as $g$. Our goal is to learn domain-invariant node representations while minimizing the error in the source domain $\epsilon_{\dS}(g,\phi)$. However, the challenge is that in the graph setting, the entries of $\mh^{(L)}$ are not independent of each other. So, it is practically impossible to view the joint distribution of node representations as a whole and align such a joint distribution across domains. The common practice to deal with this issue is to use a sampling procedure to marginalize the joint distribution:

\begin{definition}[Marginalization] For domain $\dU$, given node representations in $\mh^{(k)}$, uniformly at random sampling one of them $h_v^{(k)}$, denote the distribution of $h_v^{(k)}$ as $\mathbb{P}_{\phi}^{\dU}$.
\end{definition}

With marginalization, we consider the following objective 
\begin{equation}
    \label{eq:analysis-goal}
    \min_{g,\phi}\; \epsilon_{\dS}(g,\phi) \quad \text{s.t.} \; \mathbb{P}_{\phi}^{\dS} = \mathbb{P}_{\phi}^{\dT}.
\end{equation}

\pan{From here:} We break the GNN into two parts $\phi=\phi_{>k}\circ\phi_{\leq k}$ where $\phi_{\leq k}$ denotes the encoder of the first $k(<L)$ layers $\mh^{(k)}=\phi_{\leq k}(\mx,\mA)$ and $\mh^{(L)}=\phi_{>k}(\mh^{(k)},\mA)$. $\phi_{\leq0}$ works just as transformation of node attributes without using the graph structure.

%$\mh^{(k)}=\phi_1(\mx,\mA)$, for s$k<L$ and $\mh^{(L)}=\phi_2(\mh^{(k)},\mA)$.

\pan{Can we avoid manually enforcing invariance in the last-layer if no structure shift? We need to show as proposition 1: Suppose no structure shift $\bP_{\mA\times \mY}^\dS=\bP_{\mA\times \mY}^\dT$. Even if one aligns the marginal dis of node features $\bP^\dS_{\phi_{\leq0}}= \bP^\dT_{\phi_{\leq0}}$, there is no guarantee of $\mathbb{P}_{\phi}^{\dS} = \mathbb{P}_{\phi}^{\dT}$.}

\pan{Remark: If we align $\bP^\dS_{\phi_{\leq0}|Y}= \bP^\dT_{\phi_{\leq0}|Y}$, we have $\mathbb{P}_{\phi}^{\dS} = \mathbb{P}_{\phi}^{\dT}$. See proof in Appendix xxx. Briefly mention label shift, which will be discussed later.}

\pan{We need to show as proposition 2: Suppose we have structure shift $\bP_{\mA\times \mY}^\dS\neq\bP_{\mA\times \mY}^\dT$. We align $\mathbb{P}_{\phi}^{\dS} = \mathbb{P}_{\phi}^{\dT}$. Will aligning $\mathbb{P}_{\phi_{\leq k}}^{\dS} = \mathbb{P}_{\phi_{\leq k}}^{\dT}$ help? No... }


: Uniformly at random    

for domain $\dU\in\{\dS, \dT\}$, we denote $\mathbb{P}_{\phi}^{\dU}$ as the distribution of $\mh_{\dU}^{(L)}$, i.e., the joint distribution of node representations in domain $\dU$. 

Our goal is to learn domain-invariant node representations while minimizing the error in the source domain. 


Specifically, we consider the following objective 

\begin{equation}
    \label{eq:analysis-goal}
    \min_{g,\phi} \epsilon_{\dS}(g,\phi) \quad \text{s.t.} \; \mathbb{P}_{\phi}^{\dS} = \mathbb{P}_{\phi}^{\dT}.
\end{equation}




$\bP^\dS_{\mH}$
$\epsilon_{\dS}(g,\phi)$

%$\bP^\dS_{\mX\times\mY}\neq \bP^\dT_{\mX\times\mY}$, or equivalently $\bP^\dS_{X\times Y}\neq \bP^\dT_{X\times Y}$.



\underline{structure shift} is defined based on the joint distribution with labels, i.e. $\bP_{\mA\times \mY}^{\dS}\neq \bP_{\mA\times \mY}^{\dT} $


(given node feature then define)


for  domain $\dU\in\{\dS,\dT\}$
Attribute shift refers to $\bP^\dS_{X}\neq \bP^\dT_{X}$.

 Denote the joint distribution of node attributes $\mX^\dU$ and labels $\mY^\dU$ as $\bP^\dU_{\mX\times\mY}$ for domain $\dU\in\{\dS,\dT\}$ 

We assume without graph structure the attributes $x_v$ are IID across different nodes sampled from $\bP_{X}$. Then, the distribution $\mX^\dU$ can be written as $\prod_{v\in \dV^\dU} \bP^\dU_{X}$ where $\dU$ denotes the corresponding domain $\dU\in\{\dS,\dT\}$. Attribute shift is defined as $\bP^\dS_{X}\neq \bP^\dT_{X}$.

We assume without graph structure the attributes and label $(x_v, y_v)$ are IID across different nodes sampled from $\bP_{X\times Y}$. Then, the joint distribution of node attributes $\mX^\dU$ and node labels $\mY^\dU$ can be written as $\prod_{v\in \dV^\dU} \bP^\dU_{X\times Y}$ where $\dU$ denotes the corresponding domain $\dU\in\{\dS,\dT\}$. Attribute shift is defined as $\bP^\dS_{X\times Y}\neq \bP^\dT_{X\times Y}$.


the joint distribution of 
Consider the joint distribution of node attributes $\mX^\dU$ and node labels $\mY^\dU$ for $\dU\in\{\dS,\dT\}$.

node attributes and its label    


The general node feature shift is defined by the shift in the joint distribution of node features $X$ and node labels $Y$, that is $\mathbb{P}_{\mathcal{X}_S\times \mathcal{Y}_S} \neq \mathbb{P}_{\mathcal{X}_T\times \mathcal{Y}_T}$. This work will focus on the shift in conditional feature shift, the discussion over label shift will be left as a future direction. Then the node feature shift is expressed as $\mathbb{P}_{\mathcal{X}_S|Y_S} \neq \mathbb{P}_{\mathcal{X}_T|Y_T}$. This concept can be extended to node embeddings updated at each iteration in latent space $\mathcal{H}^{(k)}$, where $\mathbb{P}_{\mathcal{H}_S^{(k)}|Y_S} \neq \mathbb{P}_{\mathcal{H}_T^{(k)}|Y_T}$. 



Without graph-structure shift (defined later), only aligning node-feature distributions before MP is suboptimal; With graph-structure shift, aligning node representations in the intermediate layer induces information loss.

Our discussion in this subsection is on the condition that a GNN feature extractor $\phi$ can be trained to make the distributions of last-layer node representations invariant across domains, i.e.,  in Eq.~\eqref{eq:bound}, 

$\bP_{\dH^{(L)}}^\dS = \bP_{\dH^{(L)}}^\dT$


%i.e., th

Our fol two cases: Without graph-structure shift (defined later), only aligning node-feature distributions before MP is suboptimal; With graph-structure shift, aligning node representations in the intermediate layer induces information loss.

In particular, we discuss two cases with and without the graph-structure shift (defined later) across domains. We show that without 

discuss the benefits and limitations () 

In section~\ref{subsec:benefits}, we will discuss the benefit of Post-MP invariant representation learning. In section~\ref{subsec:limitation}, we will argue why Post-MP invariant representation learning is not optimal under the graph UDA problem. \pan{Not quite understand: As discussed above in section~\ref{sec:prelim}, the optimal model with minimization of target classification error should have the lowest classification with the domain-invariant representation. We already classify the common algorithms under the graph UDA problem as post-MP invariant representation learning.} Therefore, given that the domain-invariant representation has been obtained, the following analysis should focus on \textit{whether post-MP invariant representation learning can result in the lowest possible source classification error.} 

To help formulate the following analysis, we characterize the lowest possible source classification error in terms of the Bayes Error Rate (BER) \pan{why?} and give our definition of distribution shifts on graphs. We define node feature shift and graph structure shift separately instead of considering the distribution shift in node embedding space $\mathcal{H}$ after the MP like in previous works. 

BER defines the lowest possible misclassification error for any classifier given the input distribution. Several bounds for BER have been proposed~\cite{chernoff1952measure, berisha2015empirically, kailath1967divergence, lin1991divergence, sekeh2020learning}. In this work, we choose the bound in terms of Jensen-Shannon Divergence (JSD). \citet{lin1991divergence} derived a bound on pairwise BER for each pair of class labels and multi-class BER with JSD. For $\mathbb{P}_\mathcal{Y} = \pi$, where $\mathbb{P}(y=i) = \pi_i$ and $\mathbb{P}_{\mathcal{X}_i} = \mathbb{P}(X|Y=i)$ for $i$ in classes $\{1, 2, \dots, m\}$. The multi-class BER $\epsilon^m$ on generalized JSD is as follows:
\begin{equation}
    \epsilon^m \leq \frac{1}{2}(H(\pi)-JS_\pi(\mathbb{P}_{\mathcal{X}_0}, \mathbb{P}_{\mathcal{X}_1}, \dots, \mathbb{P}_{\mathcal{X}_m}))
\end{equation}
\begin{equation}
    \epsilon^m \geq \frac{1}{4(m-1)}(H(\pi)-JS_\pi(\mathbb{P}_{\mathcal{X}_0}, \mathbb{P}_{\mathcal{X}_1}, \dots, \mathbb{P}_{\mathcal{X}_m}))^2
\end{equation}
where $H(\pi)$ is the Shannon entropy and $JS_\pi$ is defined as
\begin{equation}
    JS_\pi(\mathbb{P}_{\mathcal{X}_0}, \mathbb{P}_{\mathcal{X}_1}, \dots, \mathbb{P}_{\mathcal{X}_m}) = H(\sum_{i=1}^m \pi_i\mathbb{P}_{\mathcal{X}_i}) - \sum_{i=1}^m\pi_iH(\mathbb{P}_{\mathcal{X}_i})
\end{equation}
\sk{conflict with hidden space embedding vector $H_v$}
Under the graph UDA problem, the classifier $g$ is defined on the latent representation space $\mathcal{Z}$ that is learned through a shared feature extractor $\phi$ between the source and target graph. In this case, the BER is bounded by the JSD defined over conditional distributions on latent space. \pan{Why talk about this? By the data processing inequality (DPI) ~\cite{cover2012elements} that data processing will not increase the discrimination information in the data, which implies that $JS_\pi(\mathbb{P}_{\mathcal{Z}_0}^{\phi}, \dots, \mathbb{P}_{\mathcal{Z}_m}^{\phi}) \leq JS_\pi(\mathbb{P}_{\mathcal{X}_0}, \dots, \mathbb{P}_{\mathcal{X}_m})$.} In this case, BER will be higher with latent representations as input to classifiers. That is, the objective of the feature transformation function should learn the most discriminant representation by $\max_\phi JS_\pi(\mathbb{P}_{\mathcal{Z}_0}^{\phi}, \dots, \mathbb{P}_{\mathcal{Z}_m}^{\phi})$ to reach $JS_\pi(\mathbb{P}_{\mathcal{X}_0}, \dots, \mathbb{P}_{\mathcal{X}_m})$ in BER. Combined with previous domain-invariant representation, the overall model objective is \pan{I do not understand why not use the original classification error but redefine by using JS.}
\begin{equation}
    \label{eq:JSobjective}
    \max_\phi JS_\pi(\mathbb{P}_{\mathcal{Z}_{S,0}}^{\phi}, \dots, \mathbb{P}_{\mathcal{Z}_{S,m}}^{\phi}) \; \text{s.t.} \; \mathbb{P}_{\mathcal{Z}_S}^{\phi} = \mathbb{P}_{\mathcal{Z}_T}^{\phi}
\end{equation}

\textbf{Node feature shift.} The general node feature shift is defined by the shift in the joint distribution of node features $X$ and node labels $Y$, that is $\mathbb{P}_{\mathcal{X}_S\times \mathcal{Y}_S} \neq \mathbb{P}_{\mathcal{X}_T\times \mathcal{Y}_T}$. This work will focus on the shift in conditional feature shift, the discussion over label shift will be left as a future direction. Then the node feature shift is expressed as $\mathbb{P}_{\mathcal{X}_S|Y_S} \neq \mathbb{P}_{\mathcal{X}_T|Y_T}$. This concept can be extended to node embeddings updated at each iteration in latent space $\mathcal{H}^{(k)}$, where $\mathbb{P}_{\mathcal{H}_S^{(k)}|Y_S} \neq \mathbb{P}_{\mathcal{H}_T^{(k)}|Y_T}$. 

\sk{add conditional information into it and probably can use degree to be clear. the graph structure shift in the node classification task is more like an induced extra conditional shift with MP step}\\
\textbf{Graph structure shift.} Just consider one layer of MP in GNN, and suppose we have node embeddings without conditional node feature shift from the last iteration $H_v^{(k-1)}$ as inputs, where $\mathbb{P}_{\mathcal{H}_S^{(k-1)}|Y_S} = \mathbb{P}_{\mathcal{H}_T^{(k-1)}|Y_T}$. Denote MP as a permutation equivariant function $\psi$ that takes in node embeddings matrix $H$ and adjacency matrix $A$, then with a permutation matrix $P$, $\psi(PH, PAP^T)=P\psi(H, A)$. For MP on each node $v$ following Eq.~\eqref{eq:GNN}, the AGG function is permutation invariant to the order of adjacent nodes. Then, the graph structure shift exists if the resulting node embeddings $H_v^{(k)}$ are no longer domain-invariant after one-layer of MP following Eq.~\eqref{eq:GNN}, where $\mathbb{P}_{\mathcal{H}_S^{(k)}|Y_S} \neq \mathbb{P}_{\mathcal{H}_T^{(k)}|Y_T}$.  
 
\label{sec:analysis}
\subsection{Benefits of Post-MP Invariant Representation Learning}
\label{subsec:benefits}
Given our definition of node feature shift and the graph structure shift, we classify the distribution shifts on graphs into two scenarios: with graph structure shift and without graph structure shift. In the rest of this subsection, we will provide rationales over post-MP invariant representation learning under these two scenarios respectively under the objective defined as Eq.~\eqref{eq:JSobjective}.

\textbf{Without graph structure shift.} Under the case where there exists only node feature shift, in addition to the post-MP approach, we can take a pre-MP approach for invariant representation learning. In other words, we impose a $\phi_{pre}$ function to map $X_v$ to domain invariant representation $X'_v$ first, where $\mathbb{P}_{\mathcal{X'}_S}^{\phi_{pre}} = \mathbb{P}_{\mathcal{X'}_T}^{\phi_{pre}}$; and then, we generate the node embeddings with MP step in GNN. By the definition of graph structure shift, if the input representations are domain invariant, in this case, $\mathbb{P}_{\mathcal{X'}_S}^{\phi_{pre}} = \mathbb{P}_{\mathcal{X'}_T}^{\phi_{pre}}$, the resulting embedding $H'_v$ should also be domain-invariant if there is no graph structure shift. Therefore, $\mathbb{P}_{\mathcal{H'}_S}^{\phi_{pre}} = \mathbb{P}_{\mathcal{H'}_T}^{\phi_{pre}}$ can be regarded as invariant representation like $\mathbb{P}_{\mathcal{Z}_S}^\phi = \mathbb{P}_{\mathcal{Z}_T}^\phi$ in Eq.~\eqref{eq:JSobjective} with $\phi_{pre}$ and the MP. Given that we can reach invariant representation in the objective through both pre-MP and post-MP approach, then the question is: \textit{Which method can result in a larger $JS_\pi(\mathbb{P}_{\mathcal{Z}_{S,0}}^{\phi}, \dots, \mathbb{P}_{\mathcal{Z}_{S,m}}^{\phi})$?}

The answer is that the post-MP approach can provide a larger JSD between conditional distribution in latent representation. When the MP is injective~\cite{xu2018powerful}, which means the message aggregation in the neighborhood will maintain all the information that maps distinct neighborhoods to distinct node embeddings after MP. By Eq.~\eqref{eq:GNN}, $H_v^{(1)}$ will contain both original feature information $X_v$ and $X_u, u\in N(v)$ if we consider the first iteration of MP. In this case, $\phi_{pre}$ generates the invariant and discriminant latent representation only given the node feature information of each node. However, $\phi_{post}$ generates the invariant and discriminant latent representation given both the center node feature and node features aggregated from the neighborhood. Naturally, the optimal solution of the $\phi_{post}$ should upper bound the optimal solution of the $\phi_{pre}$. From the information perspective, as the MP step follows the same mechanism in each case, then the pre-MP approach indeed bounds the amount of information by introducing $\phi_{pre}$, which makes $JS_\pi(\mathbb{P}_{\mathcal{H'}_{S,0}}^{\phi_{pre}}, \dots, \mathbb{P}_{\mathcal{H'}_{S,m}}^{\phi_{pre}}) \leq JS_\pi(\mathbb{P}_{\mathcal{Z}_{S,0}}^{\phi_{post}}, \dots, \mathbb{P}_{\mathcal{Z}_{S,m}}^{\phi_{post}})$. 

\textbf{With graph structure shift.}
Still consider the one-layer of MP as in Eq.~\eqref{eq:GNN}, under graph structure shift, MP will induce the node embedding shift even when the input node embeddings are domain-invariant as defined above. In this case, we must adopt post-MP approach to ensure the final domain-invariant representation. However, GNNs always have many layers of MP in order to get the final node embeddings, and each iteration of MP will induce an additional shift in node embeddings. Certainly, it is mandatory to have post-MP invariant representation learning after all MP steps, but \textit{is it necessary to introduce a pre-post-MP approach?} Specifically, given the graph structure shift, the previous MP layer will result in $\mathbb{P}_{\mathcal{H}_S^{(k-1)}} \neq \mathbb{P}_{\mathcal{H}_T^{(k-1)}}$, then should we first generate invariant representation $\mathbb{P}_{\mathcal{H}_S^{(k-1)}} = \mathbb{P}_{\mathcal{H}_T^{(k-1)}}$ before the $k$-th layer of MP.

Our argument is that we should not generate invariant representation before the MP, rather we should only rely on the post-MP feature mapping to get invariant representation. This shares a similar idea with the analysis regarding no graph structure shift. Based on the DPI, if we add additional transformation before MP, $JS_\pi(\mathbb{P}_{\mathcal{H'}_{S,0}^{(k-1)}}^{\phi_{pre}}, \dots, \mathbb{P}_{\mathcal{H'}_{S,m}^{(k-1)}}^{\phi_{pre}}) \leq JS_\pi(\mathbb{P}_{\mathcal{H}_{S,0}^{(k-1)}}, \dots, \mathbb{P}_{\mathcal{H}_{S,m}^{(k-1)}})$. Then, after MP $H_v^{(k)}$ that takes in $H_v^{(k-1)}$ will make $JS_\pi(\mathbb{P}_{\mathcal{H'}_{S,0}^{(k)}}^{\phi_{pre}}, \dots, \mathbb{P}_{\mathcal{H'}_{S,m}^{(k)}}^{\phi_{pre}}) \leq JS_\pi(\mathbb{P}_{\mathcal{H}_{S,0}^{(k)}}, \dots, \mathbb{P}_{\mathcal{H}_{S,m}^{(k)}})$. After all, since there is no need to adopt extra feature transformation before each layer of MP, the post-MP invariant representation learning should outperform the pre-post-MP approach in terms of classification. 

We conclude that for both with and without graph structure shift, it is reasonable to get invariant representations after the MP. However, \textit{is the post-MP method optimal?}. In the next subsection, we will argue that post-MP using a shared feature transformation $\phi_{post}$ is not optimal in terms of $\max_\phi JS_\pi(\mathbb{P}_{\mathcal{Z}_{S,0}}^{\phi}, \dots, \mathbb{P}_{\mathcal{Z}_{S,m}}^{\phi})$.

\subsection{Limitations of Post-MP Invariant Representation Learning}
\sk{relate the discussion more towards the limitation in terms of handling conditional shift. More from the conditional distribution perspective}
\label{subsec:limitation}
Above we claim that the invariant representation learning should be treated as a post-MP approach, and in this section, we will point out that post-MP invariant representation learning through a shared feature extractor across the source and target graph is not sufficient by presenting an intuitive motivating example.  

\textbf{A motivating example} We can focus on the binary node classification tasks that $Y\in\{0, 1\}$. To simplify, assume that we have the source and target graph with only graph structure shift and no node feature shift. In addition, we assume the graph is generated by the Contextual Stochastic Block Model (CSBM). Under this example, we study the case that nodes are in two classes $\mathcal{C} = \{0, 1\}$ with equal probability. The graph $G = (V, E, X)$ is sampled from CSBM with parameters $(n, p, q, \mathbb{P}_{\mathcal{X}_0}, \mathbb{P}_{\mathcal{X}_1})$, where $n$ is the number of nodes. For each node $v$, the node feature is sampled from $\mathbb{P}_{\mathcal{X}_i}$, which is $\mathbb{P}(X|Y=i)$ for $i\in\{0, 1\}$. Then, for two nodes $u$ and $v$, the probability that there is an edge between them is $p$ if $y_u=y_v$; otherwise, the edge connecting probability is $q$ when $y_u\neq y_v$. The node features and edge formulations are independent given node labels. 

Here, we make the node features a fixed value and perfectly separable for nodes with labels 0 and 1. Node features are a fixed value where $X_v = 1$ for $v \in \{V|y_v = 1\}$ and $X_v = 0$ for $v \in \{V|y_v = 0\}$. Denote $\mathbb{P}_{\mathcal{X}_{U,i}}$ as $\mathbb{P}_{\mathcal{X}_i}$ for different domain $U\in\{S,T\}$ and classes $i\in\{0, 1\}$.
$$\mathbb{P}_{\mathcal{X}_{S,0}}(X) = \mathbb{P}_{\mathcal{X}_{T,0}}(X) = \begin{cases} 1 &\text{if}  \; X = 0\\
0 &  \; \text{otherwise.}
\end{cases}$$
$$\mathbb{P}_{\mathcal{X}_{S,1}}(X) = \mathbb{P}_{\mathcal{X}_{T,1}}(X) = \begin{cases} 1 &\text{if}  \; X = 1\\
0 &  \; \text{otherwise.}
\end{cases}$$

Then, following the post-MP invariant representation learning pipeline, the model will perform MP  with input source and target graph $G_S = (V_S, E_S, X_S), G_T = (V_T, E_T, X_T)$. When the MP is injective in GNN, we can think of the MP on graphs in terms of collecting a multiset of feature vectors as messages from each neighborhood. If just consider one layer of MP, the original conditional feature distributions over different classes will become new distributions that take values as multisets. Denote the obtained multiset of messages as $M_v$ with $\mathbb{P}_\mathcal{M}$. Similarly, $\mathbb{P}_{\mathcal{M}_{U, i}}$ denotes $\mathbb{P}(M|y=i)$ under domain $U\in{S, T}$. As we assume the CSBM model which has edge connecting probabilities to connect edges in the graph independently given the node labels, $\mathbb{P}_{\mathcal{M}_{U, i}}$ can be represented as binomial distribution with parameters $p_S, q_S, p_T, q_T$. This is because the message of a node $v$ is simply a composition of a certain number of node features from class 1 nodes and class 0 nodes, which are determined by two binomial distributions. For instance, suppose we have a node $v$ with $y_v=0$ from the source domain, the message after one MP of this node can be $\{0, 0, 0, 1\}$. It means that node $v$ is connected to 3 nodes in class 0 and 1 node in class 1. The probability of getting this message with a class 0 node in the source domain is: $\mathbb{P}_{\mathcal{M}_{S, 0}}(M = \{0, 0, 0, 1\}) = {n/2 \choose 3}(p_{S})^3(1-p_S)^{n/2-3} \times {n/2 \choose 1}(q_{S})(1-q_S)^{n/2-1}$. Namely, in total there are $n/2$ class 1 nodes and class 0 nodes each, and the probability of having 3 intra-class nodes as its neighbor follows the binomial distribution of drawing $n/2$ trials of Bernoulli distribution with intra-class edge connection probability $p_S$, so as the 1 inter-class nodes following the binomial distribution with parameters $(n/2, q_S)$. We can denote the message as the multiset $({\{0, 1\}, \{(0, k_0), (1, k_1)\}})$, that contains $k_0$ number of feature 0 and $k_1$ number of feature 1. Then, $\mathbb{P}_{\mathcal{M}_{U, 0}}$ and $\mathbb{P}_{\mathcal{M}_{U, 1}}$ can be expressed as 
\begin{equation}
    \begin{aligned}
        & \mathbb{P}_{\mathcal{M}_{U, 0}}(M = ({\{0, 1\}, \{(0, k_0), (1, k_1)\}}))\\
        &\quad = {n/2\choose k_0}(p_U)^{k_0}(1-p_U)^{n/2-k_0}{n/2\choose k_1}(q_U)^{k_1}(1-q_U)^{n/2-k_1}
    \end{aligned}
\end{equation}
\begin{equation}
    \begin{aligned}
        & \mathbb{P}_{\mathcal{M}_{U, 1}}(M = ({\{0, 1\}, \{(0, k_0), (1, k_1)\}}))\\
        &\quad = {n/2\choose k_0}(q_U)^{k_0}(1-q_U)^{n/2-k_0}{n/2\choose k_1}(p_U)^{k_1}(1-p_U)^{n/2-k_1}
    \end{aligned}
\end{equation}

 Next, we will argue that the post-MP invariant representation learning through a shared feature transformation $\phi_{post}$ across the source and target domain is not sufficient in terms of the JSD between $\mathbb{P}_{\mathcal{Z}_{S, 0}}^{\phi_{post}}$ and $\mathbb{P}_{\mathcal{Z}_{S, 1}}^{\phi_{post}}$. As in the post-MP approach, the feature extractor is operated on the after MP node embedding space $\mathcal{H}$ that elaborates on the message space $\mathcal{M}$ as defined above, thus there is an upper bound that $JS(\mathbb{P}_{\mathcal{Z}_{S, 0}}^{\phi_{post}}, \mathbb{P}_{\mathcal{Z}_{S, 1}}^{\phi_{post}}) < \min(JS(\mathbb{P}_{\mathcal{M}_{S, 0}}, \mathbb{P}_{\mathcal{M}_{S, 1}}), JS(\mathbb{P}_{\mathcal{M}_{T, 0}}, \mathbb{P}_{\mathcal{M}_{T, 1}}))$ given there exists distribution shifts on the graph. However, if we consider a non-shared transformation $\omega$ that is only applied to the source graph before the shared $\phi_{post}$ after the MP, there is a lower bound of that $JS(\mathbb{P}_{\mathcal{Z}_{S, 0}}^{\phi_{post}\circ \omega}, \mathbb{P}_{\mathcal{Z}_{S, 1}}^{\phi_{post}\circ \omega}) \geq \min(JS(\mathbb{P}_{\mathcal{M}_{S, 0}}, \mathbb{P}_{\mathcal{M}_{S, 1}}), JS(\mathbb{P}_{\mathcal{M}_{T, 0}}, \mathbb{P}_{\mathcal{M}_{T, 1}}))$. Clearly, if we introduce an additional operation only on the source graph to help generate the invariant representation, the source classification error will be better than the post-MP invariant learning method through a shared $\phi_{post}$. \sk{detail should be put into appendix}
 
 As motivated by this simplified example, we will detail how to design the transformation $\omega$ on the source graph and incorporate that into the training pipeline in the next section. 


==> old-004-method-i-118.tex <==
\section{Optimality of Post-GNN Domain Invariance}\label{sec:analysis}
% \pan{First give the definition of structural shift and node shift. If we do not have S-shift, when we remove shift in node features. We are always good. If we have structural shift, Intuitively, post-MP shift removal can.... However, the first question is whether shift removal could be added to non-last layer.} 

% \pan{Any benefits for pre-MP shift removal? As long as the MP satisfies injective mapping, adding one pre-MP shift removal is useless. To explain this, we want to use the notation of Eq.~\eqref{eq:GNN}. Just consider one layer. Give the theorem based on information processing inequality. Note here you probably need KL. Also, I did not clearly see whether you need label shift = 0.}

% \pan{Any limitations for just post-MP shift removal? What is the upper bound?}

In this section, we will analyze and provide the reason why only regularizing the last-layer node representations is optimal, if learning representations  with a distribution invariant across domains is set as the goal. % (Sec.~\ref{subsec:benefits}). %Then, we show that learning invariant representations is actually sub-optimal when the distributions of neighbors conditional on the node label shift across domains (Sec.~\ref{subsec:limitation}). 

\subsection{Distribution Shifts in Graph-structured Data} \label{subsec:shift-def}
For our analysis, we need to formally define distribution shifts in node classification tasks. Specifically,  
as both node attributes and graph structure are used for predictions, either of them may have a distribution shift between domains. %We formally define structure shift and attribute shift as follows.

\textbf{Structure shift.} A naive way to define structure shift is to compare the distributions of adjacent matrices $\bP^{\dS}_{\mA}$ and $\bP^{\dT}_{\mA}$ from two domains respectively. However, this does not consider the effect of node labels. So, we consider the joint distribution with node labels $\bP_{\mA\times \mY}$. As nodes are not ordered, we have $\bP_{\mA\times \mY}(\mA, \my) = \bP_{\mA\times \mY}(\mPi\mA\mPi^\top, \mPi\my)$ for any  $\mPi$. \underline{Structure shift} refers to $\bP_{\mA\times \mY}^\dS\neq\bP_{\mA\times \mY}^\dT$. %Note that this means either label shift $\bP_{\mY}^\dS \neq\bP_{\mY}^\dT$ or label-conditional structure shift. $\bP_{\mA|\mY}^\dS\neq\bP_{\mA|\mY}^\dT$.

\textbf{Attribute shift.} We assume that by not considering the graph structure, the attributes $x_v$, $v\in\dV$ are IID sampled from $\bP_{X|Y}$ given their labels $y_v$. Therefore, the conditional distribution of $\mx|\my$ satisfies $\bP_{\mX|\mY}(\mx|\my) =\prod_{v\in \dV} \bP_{X|Y}(x_v|y_v)$, which satisfies $\bP_{\mX|\mY}(\mx|\my)= \bP_{\mX|\mY}(\mPi\mx|\my)$ for any $\mPi$ such that $\mPi\my=\my$. \underline{Attribute shift} refers to $\bP^\dS_{X|Y}\neq \bP^\dT_{X|Y}$. 



We use the joint distribution to define structure shift while the conditional distribution to define attribute shift because it better aligns with practice: Graph structure models the correlation between nodes including their labels while node attributes are often independent given their labels. 

%\subsection{Optimality of Post-GNN Domain-Invariance}
%\label{subsec:benefits}
%As both node attributes and graph structure provide information for making predictions on the graph, the distribution of either of them may shift between domains, named attribute shift and structure shift, respectively,  
%which will be formally defined later. 
 %First, we define structure shift and attribute shift.

\subsection{Analysis of Domain Invariance and Observations} \label{subsec:observation}

Our analysis is built upon the error bound in Eq.~\eqref{eq:bound}. We view the  GNN as $\phi$ to transform the node attributes and the graph structure into node representations $\mh^{(L)}=\phi(\mx,\mA)$ and the downstream node classifier as $g$. Our goal is to learn domain-invariant node representations while minimizing the error in the source domain $\epsilon_{\dS}(g,\phi)$. However, the challenge is that in the graph setting, the entries of $\mh^{(L)}$ are not independent of each other. So, it is practically impossible to view the joint distribution of node representations as a whole and align such a joint distribution across domains. The common practice to deal with this issue is to use a sampling procedure to marginalize the joint distribution:

\begin{definition}[Marginalization] For domain $\dU$, given node representations $\mh^{(l)}$, marginalization is to uniformly sample one of them $h_v^{(l)}$. Denote the distribution of $h_v^{(k)}$ as $\mathbb{P}_{\phi}^{\dU}$.
\end{definition}

With marginalization, we consider the following objective 
\begin{equation}
    \label{eq:analysis-goal}
    \min_{g,\phi}\; \epsilon_{\dS}(g,\phi) \quad \text{s.t.} \; \mathbb{P}_{\phi}^{\dS} = \mathbb{P}_{\phi}^{\dT}.
\end{equation}
A comprehensive analysis should consider three scenarios (a) with only attribute shift, (b) with only structure shift, (c) with attribute + structure shifts. However, as structure shift can be transformed into a distribution shift of node representations (similar to attribute shift) after one-layer MP, we ignore case (b) by always assuming the existence of attribute shift. So, our following discussion only breaks into two cases with or without structure shift.

We break the GNN into two parts $\phi=\phi_{>l}\circ\phi_{\leq l}$ where $\phi_{\leq l}$ denotes the encoder of the first $l(<L)$ layers $\mh^{(l)}=\phi_{\leq l}(\mx,\mA)$ and $\mh^{(L)}=\phi_{>l}(\mh^{(l)},\mA)$. %For instance, denote $\phi = \phi_{>0}$ as one entire GNN encoder; denote $\phi = \phi_{>l-1}\circ \phi_{\leq l-1}$ as two composite encoders that first generates embeddings for the $L-1$ layers and then input $\mh^{(L-1)}$ to get the final $\mh^{(L)}$. 
With some abuse of notation, let $\phi_{\leq0}$ denote the first-layer transformation of node attributes before passing to the neighbors. %Our discussion mainly focuses on why the post-GNN approach $\phi = \phi_{>0}$ is optimal under the cases with and without structure shift. 

%$\mh^{(k)}=\phi_1(\mx,\mA)$, for s$k<L$ and $\mh^{(L)}=\phi_2(\mh^{(k)},\mA)$.

\iffalse
\pan{Can we avoid manually enforcing invariance in the last-layer if no structure shift? We need to show as proposition 1: Suppose no structure shift $\bP_{\mA\times \mY}^\dS=\bP_{\mA\times \mY}^\dT$. Even if one aligns the marginal dis of node features $\bP^\dS_{\phi_{\leq0}}= \bP^\dT_{\phi_{\leq0}}$, there is no guarantee of $\mathbb{P}_{\phi}^{\dS} = \mathbb{P}_{\phi}^{\dT}$. We need to give an example here.}

\pan{Remark: If we align $\bP^\dS_{\phi_{\leq0}|Y}= \bP^\dT_{\phi_{\leq0}|Y}$, we have $\mathbb{P}_{\phi}^{\dS} = \mathbb{P}_{\phi}^{\dT}$. See proof in Appendix xxx. Briefly mention label shift, which will be discussed later.}

\pan{We need to show as proposition 2: Suppose we have structure shift $\bP_{\mA\times \mY}^\dS\neq\bP_{\mA\times \mY}^\dT$. We align $\mathbb{P}_{\phi}^{\dS} = \mathbb{P}_{\phi}^{\dT}$. Will aligning $\mathbb{P}_{\phi_{\leq k}}^{\dS} = \mathbb{P}_{\phi_{\leq k}}^{\dT}$ help? No... }
\fi

% : Uniformly at random    

% for domain $\dU\in\{\dS, \dT\}$, we denote $\mathbb{P}_{\phi}^{\dU}$ as the distribution of $\mh_{\dU}^{(L)}$, i.e., the joint distribution of node representations in domain $\dU$. 

% Our goal is to learn domain-invariant node representations while minimizing the error in the source domain. 


% Specifically, we consider the following objective 

% \begin{equation}
%     \label{eq:analysis-goal}
%     \min_{g,\phi} \epsilon_{\dS}(g,\phi) \quad \text{s.t.} \; \mathbb{P}_{\phi}^{\dS} = \mathbb{P}_{\phi}^{\dT}.
% \end{equation}




% $\bP^\dS_{\mH}$
% $\epsilon_{\dS}(g,\phi)$

% %$\bP^\dS_{\mX\times\mY}\neq \bP^\dT_{\mX\times\mY}$, or equivalently $\bP^\dS_{X\times Y}\neq \bP^\dT_{X\times Y}$.



% \underline{structure shift} is defined based on the joint distribution with labels, i.e. $\bP_{\mA\times \mY}^{\dS}\neq \bP_{\mA\times \mY}^{\dT} $


% (given node feature then define)


% for  domain $\dU\in\{\dS,\dT\}$
% Attribute shift refers to $\bP^\dS_{X}\neq \bP^\dT_{X}$.

%  Denote the joint distribution of node attributes $\mX^\dU$ and labels $\mY^\dU$ as $\bP^\dU_{\mX\times\mY}$ for domain $\dU\in\{\dS,\dT\}$ 

% We assume without graph structure the attributes $x_v$ are IID across different nodes sampled from $\bP_{X}$. Then, the distribution $\mX^\dU$ can be written as $\prod_{v\in \dV^\dU} \bP^\dU_{X}$ where $\dU$ denotes the corresponding domain $\dU\in\{\dS,\dT\}$. Attribute shift is defined as $\bP^\dS_{X}\neq \bP^\dT_{X}$.

% We assume without graph structure the attributes and label $(x_v, y_v)$ are IID across different nodes sampled from $\bP_{X\times Y}$. Then, the joint distribution of node attributes $\mX^\dU$ and node labels $\mY^\dU$ can be written as $\prod_{v\in \dV^\dU} \bP^\dU_{X\times Y}$ where $\dU$ denotes the corresponding domain $\dU\in\{\dS,\dT\}$. Attribute shift is defined as $\bP^\dS_{X\times Y}\neq \bP^\dT_{X\times Y}$.


% the joint distribution of 
% Consider the joint distribution of node attributes $\mX^\dU$ and node labels $\mY^\dU$ for $\dU\in\{\dS,\dT\}$.

% node attributes and its label    


% The general node feature shift is defined by the shift in the joint distribution of node features $X$ and node labels $Y$, that is $\mathbb{P}_{\mathcal{X}_S\times \mathcal{Y}_S} \neq \mathbb{P}_{\mathcal{X}_T\times \mathcal{Y}_T}$. This work will focus on the shift in conditional feature shift, the discussion over label shift will be left as a future direction. Then the node feature shift is expressed as $\mathbb{P}_{\mathcal{X}_S|Y_S} \neq \mathbb{P}_{\mathcal{X}_T|Y_T}$. This concept can be extended to node embeddings updated at each iteration in latent space $\mathcal{H}^{(k)}$, where $\mathbb{P}_{\mathcal{H}_S^{(k)}|Y_S} \neq \mathbb{P}_{\mathcal{H}_T^{(k)}|Y_T}$. 



% Without graph-structure shift (defined later), only aligning node-feature distributions before MP is suboptimal; With graph-structure shift, aligning node representations in the intermediate layer induces information loss.

% Our discussion in this subsection is on the condition that a GNN feature extractor $\phi$ can be trained to make the distributions of last-layer node representations invariant across domains, i.e.,  in Eq.~\eqref{eq:bound}, 

% $\bP_{\dH^{(L)}}^\dS = \bP_{\dH^{(L)}}^\dT$


% %i.e., th

% Our fol two cases: Without graph-structure shift (defined later), only aligning node-feature distributions before MP is suboptimal; With graph-structure shift, aligning node representations in the intermediate layer induces information loss.

% In particular, we discuss two cases with and without the graph-structure shift (defined later) across domains. We show that without 

% discuss the benefits and limitations () 

% In section~\ref{subsec:benefits}, we will discuss the benefit of Post-MP invariant representation learning. In section~\ref{subsec:limitation}, we will argue why Post-MP invariant representation learning is not optimal under the graph UDA problem. \pan{Not quite understand: As discussed above in section~\ref{sec:prelim}, the optimal model with minimization of target classification error should have the lowest classification with the domain-invariant representation. We already classify the common algorithms under the graph UDA problem as post-MP invariant representation learning.} Therefore, given that the domain-invariant representation has been obtained, the following analysis should focus on \textit{whether post-MP invariant representation learning can result in the lowest possible source classification error.} 

% To help formulate the following analysis, we characterize the lowest possible source classification error in terms of the Bayes Error Rate (BER) \pan{why?} and give our definition of distribution shifts on graphs. We define node feature shift and graph structure shift separately instead of considering the distribution shift in node embedding space $\mathcal{H}$ after the MP like in previous works. 

% BER defines the lowest possible misclassification error for any classifier given the input distribution. Several bounds for BER have been proposed~\cite{chernoff1952measure, berisha2015empirically, kailath1967divergence, lin1991divergence, sekeh2020learning}. In this work, we choose the bound in terms of Jensen-Shannon Divergence (JSD). \citet{lin1991divergence} derived a bound on pairwise BER for each pair of class labels and multi-class BER with JSD. For $\mathbb{P}_\mathcal{Y} = \pi$, where $\mathbb{P}(y=i) = \pi_i$ and $\mathbb{P}_{\mathcal{X}_i} = \mathbb{P}(X|Y=i)$ for $i$ in classes $\{1, 2, \dots, m\}$. The multi-class BER $\epsilon^m$ on generalized JSD is as follows:
% \begin{equation}
%     \epsilon^m \leq \frac{1}{2}(H(\pi)-JS_\pi(\mathbb{P}_{\mathcal{X}_0}, \mathbb{P}_{\mathcal{X}_1}, \dots, \mathbb{P}_{\mathcal{X}_m}))
% \end{equation}
% \begin{equation}
%     \epsilon^m \geq \frac{1}{4(m-1)}(H(\pi)-JS_\pi(\mathbb{P}_{\mathcal{X}_0}, \mathbb{P}_{\mathcal{X}_1}, \dots, \mathbb{P}_{\mathcal{X}_m}))^2
% \end{equation}
% where $H(\pi)$ is the Shannon entropy and $JS_\pi$ is defined as
% \begin{equation}
%     JS_\pi(\mathbb{P}_{\mathcal{X}_0}, \mathbb{P}_{\mathcal{X}_1}, \dots, \mathbb{P}_{\mathcal{X}_m}) = H(\sum_{i=1}^m \pi_i\mathbb{P}_{\mathcal{X}_i}) - \sum_{i=1}^m\pi_iH(\mathbb{P}_{\mathcal{X}_i})
% \end{equation}
% \sk{conflict with hidden space embedding vector $H_v$}
% Under the graph UDA problem, the classifier $g$ is defined on the latent representation space $\mathcal{Z}$ that is learned through a shared feature extractor $\phi$ between the source and target graph. In this case, the BER is bounded by the JSD defined over conditional distributions on latent space. \pan{Why talk about this? By the data processing inequality (DPI) ~\cite{cover2012elements} that data processing will not increase the discrimination information in the data, which implies that $JS_\pi(\mathbb{P}_{\mathcal{Z}_0}^{\phi}, \dots, \mathbb{P}_{\mathcal{Z}_m}^{\phi}) \leq JS_\pi(\mathbb{P}_{\mathcal{X}_0}, \dots, \mathbb{P}_{\mathcal{X}_m})$.} In this case, BER will be higher with latent representations as input to classifiers. That is, the objective of the feature transformation function should learn the most discriminant representation by $\max_\phi JS_\pi(\mathbb{P}_{\mathcal{Z}_0}^{\phi}, \dots, \mathbb{P}_{\mathcal{Z}_m}^{\phi})$ to reach $JS_\pi(\mathbb{P}_{\mathcal{X}_0}, \dots, \mathbb{P}_{\mathcal{X}_m})$ in BER. Combined with previous domain-invariant representation, the overall model objective is \pan{I do not understand why not use the original classification error but redefine by using JS.}
% \begin{equation}
%     \label{eq:JSobjective}
%     \max_\phi JS_\pi(\mathbb{P}_{\mathcal{Z}_{S,0}}^{\phi}, \dots, \mathbb{P}_{\mathcal{Z}_{S,m}}^{\phi}) \; \text{s.t.} \; \mathbb{P}_{\mathcal{Z}_S}^{\phi} = \mathbb{P}_{\mathcal{Z}_T}^{\phi}
% \end{equation}

% \textbf{Node feature shift.} The general node feature shift is defined by the shift in the joint distribution of node features $X$ and node labels $Y$, that is $\mathbb{P}_{\mathcal{X}_S\times \mathcal{Y}_S} \neq \mathbb{P}_{\mathcal{X}_T\times \mathcal{Y}_T}$. This work will focus on the shift in conditional feature shift, the discussion over label shift will be left as a future direction. Then the node feature shift is expressed as $\mathbb{P}_{\mathcal{X}_S|Y_S} \neq \mathbb{P}_{\mathcal{X}_T|Y_T}$. This concept can be extended to node embeddings updated at each iteration in latent space $\mathcal{H}^{(k)}$, where $\mathbb{P}_{\mathcal{H}_S^{(k)}|Y_S} \neq \mathbb{P}_{\mathcal{H}_T^{(k)}|Y_T}$. 

% \sk{add conditional information into it and probably can use degree to be clear. the graph structure shift in the node classification task is more like an induced extra conditional shift with MP step}\\
% \textbf{Graph structure shift.} Just consider one layer of MP in GNN, and suppose we have node embeddings without conditional node feature shift from the last iteration $H_v^{(k-1)}$ as inputs, where $\mathbb{P}_{\mathcal{H}_S^{(k-1)}|Y_S} = \mathbb{P}_{\mathcal{H}_T^{(k-1)}|Y_T}$. Denote MP as a permutation equivariant function $\psi$ that takes in node embeddings matrix $H$ and adjacency matrix $A$, then with a permutation matrix $P$, $\psi(PH, PAP^T)=P\psi(H, A)$. For MP on each node $v$ following Eq.~\eqref{eq:GNN}, the AGG function is permutation invariant to the order of adjacent nodes. Then, the graph structure shift exists if the resulting node embeddings $H_v^{(k)}$ are no longer domain-invariant after one-layer of MP following Eq.~\eqref{eq:GNN}, where $\mathbb{P}_{\mathcal{H}_S^{(k)}|Y_S} \neq \mathbb{P}_{\mathcal{H}_T^{(k)}|Y_T}$.  
 
%\label{sec:analysis}
%\subsection{Benefits of Post-MP Invariant Representation Learning}
%\label{subsec:benefits}

\textbf{Without structure shift.} Under the case with only attribute shifts, we consider if the attribute shift can be handled entirely before the GNN using a transformation $\phi_{\leq 0}$. Then, two questions arise 1). When does the invariance through $\phi_{\leq 0}$ automatically imply the invariant representation after GNN without imposing invariant learning objectives on encoder $\phi_{>0}$ and 2). Given that both the pre-GNN approach with $\phi_{\leq0}$ and post-GNN approach with $\phi_{>0}$ can achieve invariant representations as in Eq.~\eqref{eq:analysis-goal}, which approach will result in a lower classification error.

\begin{proposition}
\label{prop3.2}
    Consider the source and target graphs only exhibit attribute shifts, if there is a transformation $\phi_{\leq 0}$ on the initial node attributes before the GNN that can achieve $\mathbb{P}_{\phi_{\leq 0}|Y}^\mathcal{S} = \mathbb{P}_{\phi_{\leq 0}|Y}^\mathcal{T}$, then we claim that the after-GNN marginal node embeddings will be domain invariant as  $\mathbb{P}_\phi^\mathcal{S} = \mathbb{P}_\phi^\mathcal{T}$, where $\phi = \phi_{>0}\circ\phi_{\leq 0}$ and GNN encoder $\phi_{>0}$ is not used for invariant learning.
\end{proposition}
However, in practice, conditional invariant representations may not be easy to obtain, so existing works in GDA mostly focus on marginal distribution invariant learning. In this case, we would like to point out the following remark:
\begin{remark}
    Even when there is no structure shift, the invariant representation over marginal distribution $\mathbb{P}_{\phi_{\leq 0}}^\mathcal{S} = \mathbb{P}_{\phi_{\leq 0}}^\mathcal{T}$ before GNN using $\phi_{\leq 0}$ cannot guarantee the invariant marginal representations after GNN if the GNN encoder $\phi_{>0}$ is not optimized with the invariant learning objective.
\end{remark}
Then, we present the following proposition to answer the second question raised:
\begin{proposition}
    Suppose we can rely solely on the pre-GNN invariant learning encoder $\phi_{\leq 0}$ to reach $\mathbb{P}_\phi^\mathcal{S} = \mathbb{P}_\phi^\mathcal{T}$ as a substitute of post-GNN invariant encoder $\phi_{>0}$, the post-GNN approach will result in a lower classification error as the first term in Eq.~\eqref{eq:analysis-goal}. 
\end{proposition}
See details of the remarks and propositions in the appendix, and some brief introductions to the previous models that handle conditional invariant learning can be found in sec.~\ref{subsec:struc-cond-shift}. 

\textbf{With structure shift.}
Under the structure shift as $\bP_{\mA\times \mY}^\dS\neq\bP_{\mA\times \mY}^\dT$, each iteration of GNN will induce shifts in node embeddings, so it is obvious that the GNN encoder $\phi$ should always be optimized for final invariant representations $\mathbb{P}_\phi^\dS = \mathbb{P}_\phi^\dT$. Then, we think of if it is necessary to decompose $\phi$ into $\phi_{>k} \circ \phi_{\leq k}$ which imposes additional invariant representations in the $k$-th layer. Without loss of generality, the intermediate transformation can be anywhere between the first and last layer with $0<k<L$.

We list the proposition below to answer this question and details in the appendix:
\begin{proposition}
    Consider two GNN encoders: $\phi = \phi_{>0}$ as one entire GNN encoder that outputs the final invariant representations and $\phi = \phi_{>k}\circ\phi_{\leq k}, k<L$ as two composite encoders that enforce invariant representations both in the middle of GNN layers and at the final layer, we claim the encoder $\phi = \phi_{>0}$ will result in lower classification error. 
\end{proposition}

%We conclude that for both with and without graph structure shift, it is reasonable to get invariant representations after the MP. However, \textit{is the post-MP method optimal?}. In the next subsection, we will argue that post-MP using a shared feature transformation $\phi_{post}$ is not optimal in terms of $\max_\phi JS_\pi(\mathbb{P}_{\mathcal{Z}_{S,0}}^{\phi}, \dots, \mathbb{P}_{\mathcal{Z}_{S,m}}^{\phi})$.

%\pan{We keep the next para as transition}

Above we claim that invariant node representation learning should be treated as a post-GNN approach whether structure shift exists or not. However, the 
previous analysis is based on Eq.~\eqref{eq:bound}, where the second term is entirely ignored. As shown in Fig.~\ref{}, the ground-truth labeling functions in real-world applications may be different across domains. In the next section, we formalize the problem and propose a principled algorithm to address it.  
 


==> old-004-method-i.tex <==
\section{Analyzing Post-MP Invariant Representation Learning}
\pan{First give the definition of structural shift and node shift. If we do not have S-shift, when we remove shift in node features. We are always good. If we have structural shift, Intuitively, post-MP shift removal can.... However, the first question is whether shift removal could be added to non-last layer.} 

\pan{Any benefits for pre-MP shift removal? As long as the MP satisfies injective mapping, adding one pre-MP shift removal is useless. To explain this, we want to use the notation of Eq.~\eqref{eq:GNN}. Just consider one layer. Give the theorem based on information processing inequality. Note here you probably need KL. Also, I did not clearly see whether you need label shift = 0.}

\pan{Any limitations for just post-MP shift removal? What is the upper bound?}

In section~\ref{subsec:benefits}, we will discuss the benefit of Post-MP invariant representation learning. In section~\ref{subsec:limitation}, we will argue why Post-MP invariant representation learning is not optimal under the graph UDA problem. As discussed above in section~\ref{sec:prelim}, the optimal model with minimization of target classification error should have the lowest classification with the domain-invariant representation. We already classify the common algorithms under the graph UDA problem as post-MP invariant representation learning. Therefore, given that the domain-invariant representation has been obtained, the following analysis should focus on \textit{whether post-MP invariant representation learning can result in the lowest possible source classification error.} 

To help formulate the following analysis, we characterize the lowest possible source classification error in terms of the Bayes Error Rate (BER) and give our definition of distribution shifts on graphs. We define node feature shift and graph structure shift separately instead of considering the distribution shift in node embedding space $\mathcal{H}$ after the MP like in previous works. 

BER defines the lowest possible misclassification error for any classifier given the input distribution. Several bounds for BER have been proposed~\cite{chernoff1952measure, berisha2015empirically, kailath1967divergence, lin1991divergence, sekeh2020learning}. In this work, we choose the bound in terms of Jensen-Shannon Divergence (JSD). \citet{lin1991divergence} derived a bound on pairwise BER for each pair of class labels and multi-class BER with JSD. For $\mathbb{P}_\mathcal{Y} = \pi$, where $\mathbb{P}(y=i) = \pi_i$ and $\mathbb{P}_{\mathcal{X}_i} = \mathbb{P}(X|Y=i)$ for $i$ in classes $\{1, 2, \dots, m\}$. The multi-class BER $\epsilon^m$ on generalized JSD is as follows:
\begin{equation}
    \epsilon^m \leq \frac{1}{2}(H(\pi)-JS_\pi(\mathbb{P}_{\mathcal{X}_0}, \mathbb{P}_{\mathcal{X}_1}, \dots, \mathbb{P}_{\mathcal{X}_m}))
\end{equation}
\begin{equation}
    \epsilon^m \geq \frac{1}{4(m-1)}(H(\pi)-JS_\pi(\mathbb{P}_{\mathcal{X}_0}, \mathbb{P}_{\mathcal{X}_1}, \dots, \mathbb{P}_{\mathcal{X}_m}))^2
\end{equation}
where $H(\pi)$ is the Shannon entropy and $JS_\pi$ is defined as
\begin{equation}
    JS_\pi(\mathbb{P}_{\mathcal{X}_0}, \mathbb{P}_{\mathcal{X}_1}, \dots, \mathbb{P}_{\mathcal{X}_m}) = H(\sum_{i=1}^m \pi_i\mathbb{P}_{\mathcal{X}_i}) - \sum_{i=1}^m\pi_iH(\mathbb{P}_{\mathcal{X}_i})
\end{equation}
\sk{conflict with hidden space embedding vector $H_v$}
Under the graph UDA problem, the classifier $g$ is defined on the latent representation space $\mathcal{Z}$ that is learned through a shared feature extractor $\phi$ between the source and target graph. In this case, the BER is bounded by the JSD defined over conditional distributions on latent space. By the data processing inequality (DPI) ~\cite{cover2012elements} that data processing will not increase the discrimination information in the data, which implies that $JS_\pi(\mathbb{P}_{\mathcal{Z}_0}^{\phi}, \dots, \mathbb{P}_{\mathcal{Z}_m}^{\phi}) \leq JS_\pi(\mathbb{P}_{\mathcal{X}_0}, \dots, \mathbb{P}_{\mathcal{X}_m})$. In this case, BER will be higher with latent representations as input to classifiers. That is, the objective of the feature transformation function should learn the most discriminant representation by $\max_\phi JS_\pi(\mathbb{P}_{\mathcal{Z}_0}^{\phi}, \dots, \mathbb{P}_{\mathcal{Z}_m}^{\phi})$ to reach $JS_\pi(\mathbb{P}_{\mathcal{X}_0}, \dots, \mathbb{P}_{\mathcal{X}_m})$ in BER. Combined with previous domain-invariant representation, the overall model objective is
\begin{equation}
    \label{eq:JSobjective}
    \max_\phi JS_\pi(\mathbb{P}_{\mathcal{Z}_{S,0}}^{\phi}, \dots, \mathbb{P}_{\mathcal{Z}_{S,m}}^{\phi}) \; \text{s.t.} \; \mathbb{P}_{\mathcal{Z}_S}^{\phi} = \mathbb{P}_{\mathcal{Z}_T}^{\phi}
\end{equation}

\textbf{Node feature shift.} The general node feature shift is defined by the shift in the joint distribution of node features $X$ and node labels $Y$, that is $\mathbb{P}_{\mathcal{X}_S\times \mathcal{Y}_S} \neq \mathbb{P}_{\mathcal{X}_T\times \mathcal{Y}_T}$. This work will focus on the shift in conditional feature shift, the discussion over label shift will be left as a future direction. Then the node feature shift is expressed as $\mathbb{P}_{\mathcal{X}_S|Y_S} \neq \mathbb{P}_{\mathcal{X}_T|Y_T}$. This concept can be extended to node embeddings updated at each iteration in latent space $\mathcal{H}^{(k)}$, where $\mathbb{P}_{\mathcal{H}_S^{(k)}|Y_S} \neq \mathbb{P}_{\mathcal{H}_T^{(k)}|Y_T}$. 

\sk{add conditional information into it and probably can use degree to be clear. the graph structure shift in the node classification task is more like an induced extra conditional shift with MP step}\\
\textbf{Graph structure shift.} Just consider one layer of MP in GNN, and suppose we have node embeddings without conditional node feature shift from the last iteration $H_v^{(k-1)}$ as inputs, where $\mathbb{P}_{\mathcal{H}_S^{(k-1)}|Y_S} = \mathbb{P}_{\mathcal{H}_T^{(k-1)}|Y_T}$. Denote MP as a permutation equivariant function $\psi$ that takes in node embeddings matrix $H$ and adjacency matrix $A$, then with a permutation matrix $P$, $\psi(PH, PAP^T)=P\psi(H, A)$. For MP on each node $v$ following Eq.~\eqref{eq:GNN}, the AGG function is permutation invariant to the order of adjacent nodes. Then, the graph structure shift exists if the resulting node embeddings $H_v^{(k)}$ are no longer domain-invariant after one-layer of MP following Eq.~\eqref{eq:GNN}, where $\mathbb{P}_{\mathcal{H}_S^{(k)}|Y_S} \neq \mathbb{P}_{\mathcal{H}_T^{(k)}|Y_T}$.  
 
\label{sec:analysis}
\subsection{Benefits of Post-MP Invariant Representation Learning}
\label{subsec:benefits}
Given our definition of node feature shift and the graph structure shift, we classify the distribution shifts on graphs into two scenarios: with graph structure shift and without graph structure shift. In the rest of this subsection, we will provide rationales over post-MP invariant representation learning under these two scenarios respectively under the objective defined as Eq.~\eqref{eq:JSobjective}.

\textbf{Without graph structure shift.} Under the case where there exists only node feature shift, in addition to the post-MP approach, we can take a pre-MP approach for invariant representation learning. In other words, we impose a $\phi_{pre}$ function to map $X_v$ to domain invariant representation $X'_v$ first, where $\mathbb{P}_{\mathcal{X'}_S}^{\phi_{pre}} = \mathbb{P}_{\mathcal{X'}_T}^{\phi_{pre}}$; and then, we generate the node embeddings with MP step in GNN. By the definition of graph structure shift, if the input representations are domain invariant, in this case, $\mathbb{P}_{\mathcal{X'}_S}^{\phi_{pre}} = \mathbb{P}_{\mathcal{X'}_T}^{\phi_{pre}}$, the resulting embedding $H'_v$ should also be domain-invariant if there is no graph structure shift. Therefore, $\mathbb{P}_{\mathcal{H'}_S}^{\phi_{pre}} = \mathbb{P}_{\mathcal{H'}_T}^{\phi_{pre}}$ can be regarded as invariant representation like $\mathbb{P}_{\mathcal{Z}_S}^\phi = \mathbb{P}_{\mathcal{Z}_T}^\phi$ in Eq.~\eqref{eq:JSobjective} with $\phi_{pre}$ and the MP. Given that we can reach invariant representation in the objective through both pre-MP and post-MP approach, then the question is: \textit{Which method can result in a larger $JS_\pi(\mathbb{P}_{\mathcal{Z}_{S,0}}^{\phi}, \dots, \mathbb{P}_{\mathcal{Z}_{S,m}}^{\phi})$?}

The answer is that the post-MP approach can provide a larger JSD between conditional distribution in latent representation. When the MP is injective~\cite{xu2018powerful}, which means the message aggregation in the neighborhood will maintain all the information that maps distinct neighborhoods to distinct node embeddings after MP. By Eq.~\eqref{eq:GNN}, $H_v^{(1)}$ will contain both original feature information $X_v$ and $X_u, u\in N(v)$ if we consider the first iteration of MP. In this case, $\phi_{pre}$ generates the invariant and discriminant latent representation only given the node feature information of each node. However, $\phi_{post}$ generates the invariant and discriminant latent representation given both the center node feature and node features aggregated from the neighborhood. Naturally, the optimal solution of the $\phi_{post}$ should upper bound the optimal solution of the $\phi_{pre}$. From the information perspective, as the MP step follows the same mechanism in each case, then the pre-MP approach indeed bounds the amount of information by introducing $\phi_{pre}$, which makes $JS_\pi(\mathbb{P}_{\mathcal{H'}_{S,0}}^{\phi_{pre}}, \dots, \mathbb{P}_{\mathcal{H'}_{S,m}}^{\phi_{pre}}) \leq JS_\pi(\mathbb{P}_{\mathcal{Z}_{S,0}}^{\phi_{post}}, \dots, \mathbb{P}_{\mathcal{Z}_{S,m}}^{\phi_{post}})$. 

\textbf{With graph structure shift.}
Still consider the one-layer of MP as in Eq.~\eqref{eq:GNN}, under graph structure shift, MP will induce the node embedding shift even when the input node embeddings are domain-invariant as defined above. In this case, we must adopt post-MP approach to ensure the final domain-invariant representation. However, GNNs always have many layers of MP in order to get the final node embeddings, and each iteration of MP will induce an additional shift in node embeddings. Certainly, it is mandatory to have post-MP invariant representation learning after all MP steps, but \textit{is it necessary to introduce a pre-post-MP approach?} Specifically, given the graph structure shift, the previous MP layer will result in $\mathbb{P}_{\mathcal{H}_S^{(k-1)}} \neq \mathbb{P}_{\mathcal{H}_T^{(k-1)}}$, then should we first generate invariant representation $\mathbb{P}_{\mathcal{H}_S^{(k-1)}} = \mathbb{P}_{\mathcal{H}_T^{(k-1)}}$ before the $k$-th layer of MP.

Our argument is that we should not generate invariant representation before the MP, rather we should only rely on the post-MP feature mapping to get invariant representation. This shares a similar idea with the analysis regarding no graph structure shift. Based on the DPI, if we add additional transformation before MP, $JS_\pi(\mathbb{P}_{\mathcal{H'}_{S,0}^{(k-1)}}^{\phi_{pre}}, \dots, \mathbb{P}_{\mathcal{H'}_{S,m}^{(k-1)}}^{\phi_{pre}}) \leq JS_\pi(\mathbb{P}_{\mathcal{H}_{S,0}^{(k-1)}}, \dots, \mathbb{P}_{\mathcal{H}_{S,m}^{(k-1)}})$. Then, after MP $H_v^{(k)}$ that takes in $H_v^{(k-1)}$ will make $JS_\pi(\mathbb{P}_{\mathcal{H'}_{S,0}^{(k)}}^{\phi_{pre}}, \dots, \mathbb{P}_{\mathcal{H'}_{S,m}^{(k)}}^{\phi_{pre}}) \leq JS_\pi(\mathbb{P}_{\mathcal{H}_{S,0}^{(k)}}, \dots, \mathbb{P}_{\mathcal{H}_{S,m}^{(k)}})$. After all, since there is no need to adopt extra feature transformation before each layer of MP, the post-MP invariant representation learning should outperform the pre-post-MP approach in terms of classification. 

We conclude that for both with and without graph structure shift, it is reasonable to get invariant representations after the MP. However, \textit{is the post-MP method optimal?}. In the next subsection, we will argue that post-MP using a shared feature transformation $\phi_{post}$ is not optimal in terms of $\max_\phi JS_\pi(\mathbb{P}_{\mathcal{Z}_{S,0}}^{\phi}, \dots, \mathbb{P}_{\mathcal{Z}_{S,m}}^{\phi})$.

\subsection{Limitations of Post-MP Invariant Representation Learning}
\sk{relate the discussion more towards the limitation in terms of handling conditional shift. More from the conditional distribution perspective}
\label{subsec:limitation}
Above we claim that the invariant representation learning should be treated as a post-MP approach, and in this section, we will point out that post-MP invariant representation learning through a shared feature extractor across the source and target graph is not sufficient by presenting an intuitive motivating example.  

\textbf{A motivating example} We can focus on the binary node classification tasks that $Y\in\{0, 1\}$. To simplify, assume that we have the source and target graph with only graph structure shift and no node feature shift. In addition, we assume the graph is generated by the Contextual Stochastic Block Model (CSBM). Under this example, we study the case that nodes are in two classes $\mathcal{C} = \{0, 1\}$ with equal probability. The graph $G = (V, E, X)$ is sampled from CSBM with parameters $(n, p, q, \mathbb{P}_{\mathcal{X}_0}, \mathbb{P}_{\mathcal{X}_1})$, where $n$ is the number of nodes. For each node $v$, the node feature is sampled from $\mathbb{P}_{\mathcal{X}_i}$, which is $\mathbb{P}(X|Y=i)$ for $i\in\{0, 1\}$. Then, for two nodes $u$ and $v$, the probability that there is an edge between them is $p$ if $y_u=y_v$; otherwise, the edge connecting probability is $q$ when $y_u\neq y_v$. The node features and edge formulations are independent given node labels. 

Here, we make the node features a fixed value and perfectly separable for nodes with labels 0 and 1. Node features are a fixed value where $X_v = 1$ for $v \in \{V|y_v = 1\}$ and $X_v = 0$ for $v \in \{V|y_v = 0\}$. Denote $\mathbb{P}_{\mathcal{X}_{U,i}}$ as $\mathbb{P}_{\mathcal{X}_i}$ for different domain $U\in\{S,T\}$ and classes $i\in\{0, 1\}$.
$$\mathbb{P}_{\mathcal{X}_{S,0}}(X) = \mathbb{P}_{\mathcal{X}_{T,0}}(X) = \begin{cases} 1 &\text{if}  \; X = 0\\
0 &  \; \text{otherwise.}
\end{cases}$$
$$\mathbb{P}_{\mathcal{X}_{S,1}}(X) = \mathbb{P}_{\mathcal{X}_{T,1}}(X) = \begin{cases} 1 &\text{if}  \; X = 1\\
0 &  \; \text{otherwise.}
\end{cases}$$

Then, following the post-MP invariant representation learning pipeline, the model will perform MP  with input source and target graph $G_S = (V_S, E_S, X_S), G_T = (V_T, E_T, X_T)$. When the MP is injective in GNN, we can think of the MP on graphs in terms of collecting a multiset of feature vectors as messages from each neighborhood. If just consider one layer of MP, the original conditional feature distributions over different classes will become new distributions that take values as multisets. Denote the obtained multiset of messages as $M_v$ with $\mathbb{P}_\mathcal{M}$. Similarly, $\mathbb{P}_{\mathcal{M}_{U, i}}$ denotes $\mathbb{P}(M|y=i)$ under domain $U\in{S, T}$. As we assume the CSBM model which has edge connecting probabilities to connect edges in the graph independently given the node labels, $\mathbb{P}_{\mathcal{M}_{U, i}}$ can be represented as binomial distribution with parameters $p_S, q_S, p_T, q_T$. This is because the message of a node $v$ is simply a composition of a certain number of node features from class 1 nodes and class 0 nodes, which are determined by two binomial distributions. For instance, suppose we have a node $v$ with $y_v=0$ from the source domain, the message after one MP of this node can be $\{0, 0, 0, 1\}$. It means that node $v$ is connected to 3 nodes in class 0 and 1 node in class 1. The probability of getting this message with a class 0 node in the source domain is: $\mathbb{P}_{\mathcal{M}_{S, 0}}(M = \{0, 0, 0, 1\}) = {n/2 \choose 3}(p_{S})^3(1-p_S)^{n/2-3} \times {n/2 \choose 1}(q_{S})(1-q_S)^{n/2-1}$. Namely, in total there are $n/2$ class 1 nodes and class 0 nodes each, and the probability of having 3 intra-class nodes as its neighbor follows the binomial distribution of drawing $n/2$ trials of Bernoulli distribution with intra-class edge connection probability $p_S$, so as the 1 inter-class nodes following the binomial distribution with parameters $(n/2, q_S)$. We can denote the message as the multiset $({\{0, 1\}, \{(0, k_0), (1, k_1)\}})$, that contains $k_0$ number of feature 0 and $k_1$ number of feature 1. Then, $\mathbb{P}_{\mathcal{M}_{U, 0}}$ and $\mathbb{P}_{\mathcal{M}_{U, 1}}$ can be expressed as 
\begin{equation}
    \begin{aligned}
        & \mathbb{P}_{\mathcal{M}_{U, 0}}(M = ({\{0, 1\}, \{(0, k_0), (1, k_1)\}}))\\
        &\quad = {n/2\choose k_0}(p_U)^{k_0}(1-p_U)^{n/2-k_0}{n/2\choose k_1}(q_U)^{k_1}(1-q_U)^{n/2-k_1}
    \end{aligned}
\end{equation}
\begin{equation}
    \begin{aligned}
        & \mathbb{P}_{\mathcal{M}_{U, 1}}(M = ({\{0, 1\}, \{(0, k_0), (1, k_1)\}}))\\
        &\quad = {n/2\choose k_0}(q_U)^{k_0}(1-q_U)^{n/2-k_0}{n/2\choose k_1}(p_U)^{k_1}(1-p_U)^{n/2-k_1}
    \end{aligned}
\end{equation}

 Next, we will argue that the post-MP invariant representation learning through a shared feature transformation $\phi_{post}$ across the source and target domain is not sufficient in terms of the JSD between $\mathbb{P}_{\mathcal{Z}_{S, 0}}^{\phi_{post}}$ and $\mathbb{P}_{\mathcal{Z}_{S, 1}}^{\phi_{post}}$. As in the post-MP approach, the feature extractor is operated on the after MP node embedding space $\mathcal{H}$ that elaborates on the message space $\mathcal{M}$ as defined above, thus there is an upper bound that $JS(\mathbb{P}_{\mathcal{Z}_{S, 0}}^{\phi_{post}}, \mathbb{P}_{\mathcal{Z}_{S, 1}}^{\phi_{post}}) < \min(JS(\mathbb{P}_{\mathcal{M}_{S, 0}}, \mathbb{P}_{\mathcal{M}_{S, 1}}), JS(\mathbb{P}_{\mathcal{M}_{T, 0}}, \mathbb{P}_{\mathcal{M}_{T, 1}}))$ given there exists distribution shifts on the graph. However, if we consider a non-shared transformation $\omega$ that is only applied to the source graph before the shared $\phi_{post}$ after the MP, there is a lower bound of that $JS(\mathbb{P}_{\mathcal{Z}_{S, 0}}^{\phi_{post}\circ \omega}, \mathbb{P}_{\mathcal{Z}_{S, 1}}^{\phi_{post}\circ \omega}) \geq \min(JS(\mathbb{P}_{\mathcal{M}_{S, 0}}, \mathbb{P}_{\mathcal{M}_{S, 1}}), JS(\mathbb{P}_{\mathcal{M}_{T, 0}}, \mathbb{P}_{\mathcal{M}_{T, 1}}))$. Clearly, if we introduce an additional operation only on the source graph to help generate the invariant representation, the source classification error will be better than the post-MP invariant learning method through a shared $\phi_{post}$. \sk{detail should be put into appendix}
 
 As motivated by this simplified example, we will detail how to design the transformation $\omega$ on the source graph and incorporate that into the training pipeline in the next section. 


==> old-005-method-ii.tex <==
\section{The Structural Re-weighting Algorithms}

In this section, we first introduce the issue of structure conditional shift which emerges in many real-world node classification tasks. Then, we propose the structural re-weighting algorithm \proj to address this distribution shift.   

In this section, we will present our designed framework with edge-reweighting on the source graph inspired by the analysis in the last section~\ref{sec:analysis}. We will first introduce the motivation of the edge-reweighting method, followed by the detailed approach in section~\ref{subsec:detailrw} and overall training pipeline in section~\ref{subsec:pipeline}.

\subsection{The Issue of Structure Conditional Shift}
%\sk{relate the discussion more towards the limitation in terms of handling conditional shift. More from the conditional distribution perspective}
\label{subsec:limitation}

  In this section, we will point out that post-MP invariant representation learning through a shared feature extractor across the source and target graph is not sufficient by presenting an intuitive motivating example.

\textbf{A motivating example} We can focus on the binary node classification tasks that $Y\in\{0, 1\}$. To simplify, assume that we have the source and target graph with only graph structure shift and no node feature shift. In addition, we assume the graph is generated by the Contextual Stochastic Block Model (CSBM). Under this example, we study the case that nodes are in two classes $\mathcal{C} = \{0, 1\}$ with equal probability. The graph $G = (V, E, X)$ is sampled from CSBM with parameters $(n, p, q, \mathbb{P}_{\mathcal{X}_0}, \mathbb{P}_{\mathcal{X}_1})$, where $n$ is the number of nodes. For each node $v$, the node feature is sampled from $\mathbb{P}_{\mathcal{X}_i}$, which is $\mathbb{P}(X|Y=i)$ for $i\in\{0, 1\}$. Then, for two nodes $u$ and $v$, the probability that there is an edge between them is $p$ if $y_u=y_v$; otherwise, the edge connecting probability is $q$ when $y_u\neq y_v$. The node features and edge formulations are independent given node labels. 

Here, we make the node features a fixed value and perfectly separable for nodes with labels 0 and 1. Node features are a fixed value where $X_v = 1$ for $v \in \{V|y_v = 1\}$ and $X_v = 0$ for $v \in \{V|y_v = 0\}$. Denote $\mathbb{P}_{\mathcal{X}_{U,i}}$ as $\mathbb{P}_{\mathcal{X}_i}$ for different domain $U\in\{S,T\}$ and classes $i\in\{0, 1\}$.
$$\mathbb{P}_{\mathcal{X}_{S,0}}(X) = \mathbb{P}_{\mathcal{X}_{T,0}}(X) = \begin{cases} 1 &\text{if}  \; X = 0\\
0 &  \; \text{otherwise.}
\end{cases}$$
$$\mathbb{P}_{\mathcal{X}_{S,1}}(X) = \mathbb{P}_{\mathcal{X}_{T,1}}(X) = \begin{cases} 1 &\text{if}  \; X = 1\\
0 &  \; \text{otherwise.}
\end{cases}$$

Then, following the post-MP invariant representation learning pipeline, the model will perform MP  with input source and target graph $G_S = (V_S, E_S, X_S), G_T = (V_T, E_T, X_T)$. When the MP is injective in GNN, we can think of the MP on graphs in terms of collecting a multiset of feature vectors as messages from each neighborhood. If just consider one layer of MP, the original conditional feature distributions over different classes will become new distributions that take values as multisets. Denote the obtained multiset of messages as $M_v$ with $\mathbb{P}_\mathcal{M}$. Similarly, $\mathbb{P}_{\mathcal{M}_{U, i}}$ denotes $\mathbb{P}(M|y=i)$ under domain $U\in{S, T}$. As we assume the CSBM model which has edge connecting probabilities to connect edges in the graph independently given the node labels, $\mathbb{P}_{\mathcal{M}_{U, i}}$ can be represented as binomial distribution with parameters $p_S, q_S, p_T, q_T$. This is because the message of a node $v$ is simply a composition of a certain number of node features from class 1 nodes and class 0 nodes, which are determined by two binomial distributions. For instance, suppose we have a node $v$ with $y_v=0$ from the source domain, the message after one MP of this node can be $\{0, 0, 0, 1\}$. It means that node $v$ is connected to 3 nodes in class 0 and 1 node in class 1. The probability of getting this message with a class 0 node in the source domain is: $\mathbb{P}_{\mathcal{M}_{S, 0}}(M = \{0, 0, 0, 1\}) = {n/2 \choose 3}(p_{S})^3(1-p_S)^{n/2-3} \times {n/2 \choose 1}(q_{S})(1-q_S)^{n/2-1}$. Namely, in total there are $n/2$ class 1 nodes and class 0 nodes each, and the probability of having 3 intra-class nodes as its neighbor follows the binomial distribution of drawing $n/2$ trials of Bernoulli distribution with intra-class edge connection probability $p_S$, so as the 1 inter-class nodes following the binomial distribution with parameters $(n/2, q_S)$. We can denote the message as the multiset $({\{0, 1\}, \{(0, k_0), (1, k_1)\}})$, that contains $k_0$ number of feature 0 and $k_1$ number of feature 1. Then, $\mathbb{P}_{\mathcal{M}_{U, 0}}$ and $\mathbb{P}_{\mathcal{M}_{U, 1}}$ can be expressed as 
\begin{equation}
    \begin{aligned}
        & \mathbb{P}_{\mathcal{M}_{U, 0}}(M = ({\{0, 1\}, \{(0, k_0), (1, k_1)\}}))\\
        &\quad = {n/2\choose k_0}(p_U)^{k_0}(1-p_U)^{n/2-k_0}{n/2\choose k_1}(q_U)^{k_1}(1-q_U)^{n/2-k_1}
    \end{aligned}
\end{equation}
\begin{equation}
    \begin{aligned}
        & \mathbb{P}_{\mathcal{M}_{U, 1}}(M = ({\{0, 1\}, \{(0, k_0), (1, k_1)\}}))\\
        &\quad = {n/2\choose k_0}(q_U)^{k_0}(1-q_U)^{n/2-k_0}{n/2\choose k_1}(p_U)^{k_1}(1-p_U)^{n/2-k_1}
    \end{aligned}
\end{equation}

 Next, we will argue that the post-MP invariant representation learning through a shared feature transformation $\phi_{post}$ across the source and target domain is not sufficient in terms of the JSD between $\mathbb{P}_{\mathcal{Z}_{S, 0}}^{\phi_{post}}$ and $\mathbb{P}_{\mathcal{Z}_{S, 1}}^{\phi_{post}}$. As in the post-MP approach, the feature extractor is operated on the after MP node embedding space $\mathcal{H}$ that elaborates on the message space $\mathcal{M}$ as defined above, thus there is an upper bound that $JS(\mathbb{P}_{\mathcal{Z}_{S, 0}}^{\phi_{post}}, \mathbb{P}_{\mathcal{Z}_{S, 1}}^{\phi_{post}}) < \min(JS(\mathbb{P}_{\mathcal{M}_{S, 0}}, \mathbb{P}_{\mathcal{M}_{S, 1}}), JS(\mathbb{P}_{\mathcal{M}_{T, 0}}, \mathbb{P}_{\mathcal{M}_{T, 1}}))$ given there exists distribution shifts on the graph. However, if we consider a non-shared transformation $\omega$ that is only applied to the source graph before the shared $\phi_{post}$ after the MP, there is a lower bound of that $JS(\mathbb{P}_{\mathcal{Z}_{S, 0}}^{\phi_{post}\circ \omega}, \mathbb{P}_{\mathcal{Z}_{S, 1}}^{\phi_{post}\circ \omega}) \geq \min(JS(\mathbb{P}_{\mathcal{M}_{S, 0}}, \mathbb{P}_{\mathcal{M}_{S, 1}}), JS(\mathbb{P}_{\mathcal{M}_{T, 0}}, \mathbb{P}_{\mathcal{M}_{T, 1}}))$. Clearly, if we introduce an additional operation only on the source graph to help generate the invariant representation, the source classification error will be better than the post-MP invariant learning method through a shared $\phi_{post}$. \sk{detail should be put into appendix}
 
 As motivated by this simplified example, we will detail how to design the transformation $\omega$ on the source graph and incorporate that into the training pipeline in the next section. 



Follow the analysis in section~\ref{sec:analysis}, we conclude that the overall model should contain an additional transformation function $\omega$ only on the source graph in addition to the post-MP invariant representation learning using a shared $\phi_{post}$ and the classification function $g$. However, the choice of the function $\omega$ cannot be arbitrary mapping which potentially makes the model overfit to the source graph and cannot generalize to the target graph. Inspired by the example in section~\ref{subsec:limitation}, we design the transformation as manipulation on the source graph structure to remove the graph structure shift in order to increase the upper bound of $JS_\pi(\mathbb{P}_{\mathcal{Z}_{S,0}}^{\phi_{post}}, \dots, \mathbb{P}_{\mathcal{Z}_{S,m}}^{\phi_{post}})$. 

Actually, some real-world node classification problems may further have label-distribution shifts according to the terminology in~\cite{zhang2013domain} because the node-label-distributions may be also different across domains. However, as the node-label-distribution shift may happen or not happen in practice, and is not the focus of this work, we uniformly call the issue \emph{conditional shift} later on.

\textbf{Conditional Shift.} %\pan{Review: Some works have studied conditional shift while not for graph-structured data~\cite{zhang2013domain, zhao2019learning,tachet2020domain} (and I think there are more works). Summarize the key ideas of the group of these works. However, these methods all assume that samples are independent and cannot deal with the graph connections between samples. }
However, only learning representations invariant across the source and target domains may fail in some cases where there exists a conditional shift or label shift. The definition over the conditional shift in~\cite{zhang2013domain}, where $\mathbb{P}_{X|Y}$ changes across domains with the same marginal label distribution $\mathbb{P}_Y$, inspires works that handle conditional distribution shift~\cite{gong2016domain, long2018conditional}. \citet{long2018conditional} aligns conditional distribution through inputting conditioned representation $Z\bigotimes \hat{Y}$ into the domain discriminator. Regarding the label shift issue, it was proved that invariant marginal representation would increase the target error when the marginal label distribution $\mathbb{P}_Y^\mathcal{S}$ and $\mathbb{P}_Y^\mathcal{T}$ are significantly different~\cite{zhao2019learning, tachet2020domain, wu2019domain, azizzadenesheli2019regularized}. They further elaborated the original generalization bound of target error $\epsilon_T$ in terms of the distance between $\mathbb{P}_Y^\mathcal{S}$ and $\mathbb{P}_Y^\mathcal{T}$ by requiring the model to satisfy $\mathbb{P}_{Z|Y}^\mathcal{S} = \mathbb{P}_{Z|Y}^\mathcal{T}$. 
Therefore, the designed algorithms adopted importance weights $w_y = \frac{\mathbb{P}^\mathcal{T}(Y=y)}{\mathbb{P}^\mathcal{S}(Y=y)}, \forall y \in \mathcal{Y}$ to let $\mathbb{P}^\mathcal{T}(Z) = \sum_{y\in\mathcal{Y}}w_y\cdot\mathbb{P}^\mathcal{S}(Z, Y=y)$ in order to achieve invariant conditional representations. 
However, these previous methods all deals with the conditional shift in independent data and thus cannot handle the interdependent graph-structured samples. 

AdaGIn~\cite{xiao2022domain} adopts the graph infomax to encode global structural information together with conditional adversarial networks for invariant node representation.


\subsection{Edge re-weighting on source graphs}
\label{subsec:detailrw}

Generally, unlike node feature space, it is complicated to rigorously define the matching in terms of the graph structure. We view this problem with respect to our definition of graph structure shift. It can be inferred that the source and target graph structures are equivalent if the application of a single layer of MP results in output node embeddings that are domain-invariant, given invariant input node embeddings. Then, from the more fundamental point of view, the node embeddings $H_v$ after the MP is generated based on the messages $M_v$ aggregated in the neighborhood as described in section~\ref{subsec:limitation}. Each feature vector contained in the multiset of messages is sampled based on the edge connection probability $p, q$ defined in the CSBM model as $(n, p, q, \mathbb{P}_{\mathcal{X}_0}, \dots,  \mathbb{P}_{\mathcal{X}_m})$, and each message is a sample from the message distribution $\mathbb{P}_{\mathcal{M}_i}$ of that particular class $i$. Under this setting, message distribution is the distribution that takes values of each multiset with probability determined by the edge connections in each neighborhood. When there exists graph structure shift that causes the $\mathbb{P}_{\mathcal{M}_{S, i}} \neq \mathbb{P}_{\mathcal{M}_{T, i}}$, the primary technique should be upsampling and downsampling to make the distribution aligned. For instance, under the context of the previous motivating example in section~\ref{subsec:limitation}, $\mathbb{P}_{\mathcal{M}_{S, 0}}$ has an expected message $\{0, 1\}$ and $\mathbb{P}_{\mathcal{M}_{T, 0}}$ has an expected message $\{0, 0, 1\}$. In this case, we should upsample twice the class 0 nodes with feature 0 in the source graph to form the new message distribution $\mathbb{P}_{\mathcal{M'}_{S, 0}}$ to achieve $\mathbb{P}_{\mathcal{M'}_{S, 0}} = \mathbb{P}_{\mathcal{M}_{T, 0}}$. 

By dissecting the MP in GNN to the essential formulation of the message and reasoning that sampling over neighborhood features is the fundamental technique to align distribution over messages, we extend this idea to the general GNN setting with message pooling to form resulting node embeddings. In GNN formulation as in Eq.~\eqref{eq:GNN}, the AGG function is often set to be some pooling function, like sum/mean pooling. Namely, the AGG function aggregates the multiset function in some designed way and forms a message vector on top of that. If the previous resampling directly deals with the initial message distribution over multisets, we can elaborate on this idea to edge-reweighting when pooling the features from the multisets to form the message vector. One can think of adding weight toward the edges connected to a particular type of feature as upsampling that particular node and vice versa. 

\sk{continue from here}
In this work, the edge-reweighting method is inspired by the formulation of CSBM as introduced above, and the weights used to reweight the edges are calculated based on the edge connection probability. Denote $w_{ij}$ as the weight to add on edges connecting nodes with label $i$ and nodes with label $j$. All the weights are calculated with the matrix $B_s$ and $B_t$ from the source and target graph. We first approximate matrix $B_s$ and $B_t$, then calculate the weights $w_{ij}$ to match $B_s$ to $B_t$.

If we have class labels for each node, then matrix $B$ can be easily approximated, where $$b_{ij} = \frac{|\{e_{uv}\in E |y_u = i, y_v = j\}|}{|\{v\in V |y_v = i\}|\times |\{v\in V |y_v = j\}|}$$ We only use the node labels available in training sets for the source graph estimation. Since we do not know the node labels under the UDA setting for the target graph, we use pseudo-labels $\hat{Y}_T$ obtained through the source model by $\hat{Y}_T = g(Z_T)$, where $Z_T = \phi_{post}(H_T)$ and $H_T$ is the node embedding after the GNN.   

\subsection{Overall training pipeline}
\label{subsec:pipeline}
After detailing the edge reweighting module as our designed control for reducing graph structure shift, we will present our overall training pipeline in this section.
\sk{add pseudo-code and the paragraph saying that this method can also work on some OOD algorithms}


==> old-006-experiments.tex <==
\section{Experiments}
\label{sec:exp}
In this section, we evaluate \proj combined with for adaptation and generalization ability by comparing it with some existing GDA and Graph OOD baselines. The experiments are done on one synthetic dataset, one real dataset from HEP scientific applications and three common citation networks under various types of domain shifts. We will introduce the datasets, baselines, and experiment settings in the rest of this section. More details can be found in Appendix.

%\begin{comment}
%\sk{numbers are not correct, will fill in}
\begin{table*}[t]
\vspace{-2mm}
\caption{Synthetic CSBM results}
\vspace{-0.1cm}
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccccc}
\toprule
  &   $q=0.16$                 &    $q=0.14$                &      $q=0.12$             & $q=0.1$                  & $q=0.06$                  & $q=0.01$                  \\
\midrule
ERM & $37.69\pm4.96$ & $40.85\pm6.4$ & $47.38\pm5.73$ & $58.65\pm4.45$ & $90.49\pm2.4$ & $100\pm0$ \\
DANN  & $65.21\pm6.76$ & $71.72\pm9.36$ & $78.90\pm7.16$ & $85.00\pm9.53$ & $96.40\pm1.24$ & $99.96\pm0.06$ \\
CDAN    &  &  &  &  &  &  \\
UDAGCN          & $50.93\pm0.96$ & $56.55\pm2.91$ & $58.37\pm0.42$ & $63.37\pm0.23$ & $\mathbf{98.63}\pm0.53$ & $100\pm0$ \\
EERM          & $56.53\pm3.43$ & $64.49\pm2.75$ & $69.96\pm14.34$ & $71.47\pm15.98$ & $94.53\pm5.37$ & $100\pm0$ \\
Mixup          & $61\pm3.63$ & $68.08\pm1.12$ & $74.19\pm1.36$ & $81.93\pm2.35$ & $96.33\pm0.11$ & $100\pm0$ \\
\midrule
\projerm \\
\projad    & $\underline{85.43}^\dagger\pm4.82$ & $\underline{88.21}^\dagger\pm1.73$ & $\underline{90.36}^\dagger\pm2.04$ & $\underline{93.38}^\dagger\pm1.21$ & $98.39^\dagger\pm0.32$ & $\mathbf{100}\pm0$ \\
\projmix    & $\mathbf{88.52}^\dagger\pm1.7$ & $\mathbf{89.59}^\dagger\pm1.22$ & $\mathbf{91.81}^\dagger\pm1.03$ & $\mathbf{94.48}^\dagger\pm0.74$ & $\underline{98.59}^\dagger\pm0.13$ & $\mathbf{100}\pm0$ \\

\bottomrule
\label{table:CSBM}
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vspace{-9mm}
\end{table*}


\begin{table*}[t]
\vspace{-2mm}
\caption{OOD citation datasets}
\vspace{-0.1cm}
\begin{center}
\begin{adjustbox}{width=1\textwidth}
\begin{small}
\begin{sc}
\begin{tabular}{lcccccccc}
\toprule
  & \multicolumn{2}{c}{DBLP\&ACM} & \multicolumn{2}{c}{Cora} &   \multicolumn{4}{c}{Arxiv}\\
   & $A\rightarrow D$ & $D\rightarrow A$ &   Word &  Degree  &     time1     &      time2             & time3     & Degree       \\
\midrule
ERM & $61.08\pm0.66$ &$67.98\pm0.47$ & $\underline{67.44}\pm0.9$ & $61.67\pm0.3$ & $\underline{26.86}\pm0.33$ & $38.53\pm0.98$ & $48.66\pm0.10$ & $58.87\pm0.29$\\
DANN  & $\underline{64.00}\pm4.61$ & $64.36\pm1.16$ & $61.93\pm 2.12$ &  &  &  &  \\
CDAN    & & & & & \\
UDAGCN  &$59.59\pm1.69$ &$63.74\pm2.71$ &$64.44\pm2.26$ & $60.61\pm0.21$ & $25.26\pm5.23$ & $39.14\pm1.34$ & $47.77\pm18.25$ & $55.08\pm0.83$\\
EERM         & $36.01\pm 9.83$& $\mathbf{82.9}\pm 4.56$ & $67.28\pm2.01$ & $60.56\pm1.99$ & OOM & OOM & OOM & OOM \\
MIXUP         & $49.26\pm0.56$ &$63.9\pm0.25$ & $66.5\pm0.79$ & $60.59\pm0.64$ & $26.55\pm1.39$ & $38.41\pm1.2$ & $50.16\pm0.59$ & $58.42\pm0.64$\\
\midrule
\projerm & $62.08\pm0.74$ & $68.13\pm1.33$ & $\mathbf{67.58}\pm 0.73$ &$\mathbf{62.51}^\dagger\pm0.38$ & $\mathbf{28.32}^\dagger\pm0.67$ & $\underline{38.74}\pm0.64$ &  $\underline{48.91}\pm0.37$ & $\underline{60.04}^\dagger\pm0.38$\\
\projad & $\mathbf{67.05}^\dagger\pm 2.97$ & $\underline{68.87}^\dagger\pm3.35$ & $62.5\pm 1.91$ & &&&&\\
\projmix    & $49.32\pm0.5$ & $66.10^\dagger\pm1.2$ & $66.92\pm0.77$ &$\underline{61.92}^\dagger\pm0.37$ & $26.29\pm1.29$ & $\mathbf{39.16}\pm1.4$ & $\mathbf{50.39}^\dagger\pm0.20$ & $\mathbf{60.05}^\dagger\pm0.43$ \\

\bottomrule
\label{table:real}
\end{tabular}
\end{sc}
\end{small}

\end{adjustbox}
\end{center}
\vspace{-9mm}
\end{table*}

\begin{table*}[t]
\caption{Pileup Mitigation Datasets}
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccccc}
\toprule
  & \multicolumn{4}{c}{PU level} &  \multicolumn{2}{c}{PU level}\\
  &   $\text{PU}30 \rightarrow 10$    & $\text{PU}10 \rightarrow 30$ & PU$140\rightarrow 50$ & PU$50\rightarrow 140$ & Sig1 $\rightarrow$ Sig2      &    Sig2 $\rightarrow$ Sig1     \\
\midrule
ERM & $68.32\pm0.53$ & $69.64\pm0.62$ &$68.27\pm0.67$ & $68.95\pm 0.083$& $67.95\pm0.44$ & $67.5\pm0.98$ \\
DANN  & $69.18\pm0.60$ & $\mathbf{70.96}\pm0.48$ & $68.70\pm 0.32$ & $69.01\pm 0.95$& $70.34\pm0.41$ & $71.28\pm0.67$ \\
\midrule
\projerm & & & $68.84\dagger\pm0.46$\\
\projad    & $\mathbf{69.87}\dagger\pm0.58$ & $70.87\pm0.64$ &$\mathbf{69.12}\pm 0.64$ & $\mathbf{69.39}\pm0.63$& $\textbf{70.75}\pm0.66$& $\textbf{71.40}\pm0.26$ \\

\bottomrule
\label{table:Pileup}
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vspace{-9mm}
\end{table*}

%\end{comment}
\sk{Details will be put into appendix, will trim this part}
\subsection{Datasets}
\textbf{Synthetic CSBM} Following the def.~\ref{def:CSBM}, we construct the synthetic graphs with the CSBM model with parameters $n, \mB, \mathbb{P}_0, \dots \mathbb{P}_{k-1}$. We consider the 3-class classification problem, where both the source and target nodes are equivalently divided into 3 blocks representing each class ${0, 1, 2}$. We assume there is no attribute shift but only the structure shift as we aim to demonstrate the effectiveness of our \proj specifically under the existence of CSS. The node features are constructed by 2-dimensional gaussian distribution with $\mathbb{P}_0 = \dN([-1, 0], \Sigma), \mathbb{P}_1 = \dN([1, 0], \Sigma), \mathbb{P}_2 = \dN([3, 2], \Sigma)$. In addition, we have the $2\times 2$ matrix $\mB^\dS$ and $\mB^\dT$ for the source and target graphs respectively. We simplify the parameters in $\mB$ into $b_{ii} = b_{jj} = p$ that stands for the intra-class edge connecting probability and the $b_{ij} = b_{ji} = q$ that stands for the inter-class edge connecting probability. During the synthetic experiments, we keep the $p$ the same and vary $q$ to create the CSS between the source and target graphs.

\textbf{DBLP and ACM} are two paper citation networks obtained from DBLP and ACM respectively. Each node represents a paper, and the graph is constructed based on the citation relations, where the edge indicates a citation between two papers. The classification task is regarding the research topics, including "Database", "Data mining", "Artificial Intelligence" and so on. The DA problem is to train on citation graph from one source and test on the other, in which we will have $D\rightarrow A$ and $A \rightarrow D$. The original datasets are provided by ArnetMiner~\cite{tang2008arnetminer} and the processed version is adopted from~\cite{wu2020unsupervised}. 

\textbf{GOOD-Arxiv} is a graph representing the citation network between all Computer Science (CS) Arxiv papers. Each node is an Arxiv paper and the edge between two papers indicates that one paper cites the other, which appears to be directed. The features are embeddings of words in the title and abstract. The classification task is a 40-class classification on different subject areas. The domain can be split based on publication time and node degree and we conduct experiments on both types of splits. For the time domain shift, we keep the testing dataset to be papers published between 2018 to 2020 with varying time period for training samples. Time 1 corresponds to papers from 2005 to 2007; time 2 is from 2008 to 2010 and time 3 is from 2011 to 2014. The degree split is based on the node degrees as introduced in~\cite{gui2022good}. It is originally introduced in OGB~\cite{hu2020open} and also used as a benchmark dataset in~\cite{gui2022good}

\textbf{GOOD-Cora} is a citation dataset obtained from the full Cora dataset~\cite{bojchevski2017deep} and has been benchmarked in~\cite{gui2022good}. Similarly, the nodes are papers from scientific publications and the edges are citation relations. It is a 70-class classification problem with identifying the publication type of each paper. The domain splits are word and degree. The word split is based on the diversity of words of a publication and the degree split is based on the node degree. 

\textbf{HEP datasets} are scientific datasets from one real HEP application called pileup mitigation. They are synthetic datasets generated following some physics principles by domain experts. The nodes in the graph are particles during the collisions in the large hadron collider. As mentioned in the introduction, the task is a binary node classification problem aiming at identifying nodes from LC as opposed to OC. The distribution shift may come from two sources, the change between the signals for data generation (the change of underlying principle for data generation) and the change of physics condition (mostly the ratio between OC and LC during generation). 

\subsection{Baselines and Settings}
\textbf{Baselines} As discussed, our method \proj can be regarded as an additional module that handles CSS and therefore can be combined with existing baselines. We choose popular algorithms DANN~\cite{ganin2016domain} and Mixup ~\cite{wang2021mixup} from DA and OOD tasks together with the basic ERM using GNN as encoders. Specifically, the scores included in the table use GCN~\cite{kipf2016semi} as the backbone in order to fairly compare with baselines. For instance, the UDAGCN baseline and Mixup for graph baselines only has implementation over GCN, so we stick with their own original implementations for comparisons. However, we also explored GraphSAGE~\cite{hamilton2017inductive} and demonstrated that our \proj does not limit to specific GNN backbones. For existing GDA and GOOD works, we adopt UDAGCN~\cite{wu2020unsupervised} and EERM~\cite{wu2022handling} as baselines. However, we only include ERM and DANN as our baselines for the HEP datasets since the training and testing settings are multigraph settings, which tend to be different from existing works. We will leave this exploration in our future work. 

\textbf{Settings and Metric.}
Given the distribution shifts introduced in the datasets section, we split the datasets into source training, source testing, target training, and target testing dataset. For the datasets with multiple training and testing graphs, like the pileup dataset, we have separated graphs for each of the four categories. For the datasets with a single graph for training and testing, the splits are done through node masking. The model is trained given the source training dataset and target training dataset with the DA models like DANN, CDAN, UDAGCN, and our \proj. For the OOD baselines like EERM and Mixup, the training is done with the source training dataset. For testing, all the algorithms are tested on the same hold-out target testing dataset. 

All the evaluations are based on the accuracy score for the node classification tasks on the target testing dataset. We expect the model trained with labeled source and unlabeled target data to have satisfying target performance. The report of the final score is not selected during the training process using target validation since we are not able to access the target labels during training under the UDA setting. We report the target testing scores based on the model we get at the end of the training.  

\subsection{Experiment results}
We first demonstrate some experiments over the CSBM synthetic datasets in table~\ref{table:CSBM} to prove the effectiveness of our algorithm design. For the synthetic datasets on CSBM, we vary the inter-class connection probability $q$ in the target domain to create a series of graph distributions from the smallest to the largest while keeping the intra-class connection probability $p$ and node features the same across the domains. Under the decay of performance caused by structure shift shown in the ERM scores in the first row, \proj shows its significant improvement over the baselines without explicit handle over the graph structure that causes CSS. The models with \proj appear to be significantly higher than the baselines among all choices of inter-class probability for target graphs. Also, we notice the effectiveness of additional \proj increases with the degree of structure shift. Particularly, \proj is able to boost the performance more when the structure shift is large as in former columns. If the structure shift is originally small when $q$ is small in this case, the amount of boost is relatively small compared to the previous cases. The potential room of improvement for our \proj is naturally small, but we can still observe a better performance over the baselines. We find this result to be reasonable and match our intuition. 

The table~\ref{table:real} includes the results for three real-world citation datasets. For nearly all the datasets, one of our three models from \projerm, \projad and \projmix outperforms the other models tested. And if we closely compare the performance with the addition of our \proj to the corresponding baseline, it has been shown that \proj will achieve at least comparable performance and marginal benefits over the baselines and will gain significant improvements (difference in mean > 1 std of our model) under the case where CSS is large. For instance, our model demonstrates considerable performance under the node degree shift in Cora and Arxiv datasets compared to the word split. This indeed verifies the contribution of our \proj as to handling the structure shift induced in the graph, which aligns with the setting of node degree shift. Also, for the previous  DBLP and ACM datasets under the DA setting adopted from~\cite{wu2020unsupervised}, the \projad tends to have significant performance. Regarding the other domain splits scenarios, it is natural that the distribution shift mostly arises from the attribute level and the original ERM scores tend to be satisfying. In these cases, our model can still achieve marginal improvement (difference in mean >0.5 std of our model)over the well-studied baselines. This also verifies that our \proj will not fail given the real scenarios with mostly attribute shifts.  

Finally, regarding the HEP datasets, we basically compare the with \proj pipelines with corresponding baselines that are suitable for the setting as ERM and DANN. Under the domain shift caused by different PU levels, we have observed some significant improvements over the case adapting from the higher PU levels to lower PU levels. For the case with training on lower PU levels and testing on higher PU levels demonstrate marginal improvements. These particular results agree with previous findings in the HEP application study, where the model learned with low PU levels tends to be more robust. The signal adaptation also has some improvements over baselines but naturally encodes less degree of CSS across two domains. 

\subsection{Hyperparameter}
Other than the normal hyperparameter tuning like learning rate, model architecture and epoch as some basic setups. Our \proj basically relies on three hyperparameters: the epoch to start \proj, the frequency of calculating weights, and the $\lambda$ stands for the degree we want to adopt the reweighted message. Since the approach is based on pseudo-labels we get for the target nodes, the quality of the pseudo-labels are important. Also, the original shift in CSS will determine how much the model want to reply on the reweighted message as determined by $\lambda*h + (1-\lambda)* RW(h)$. This can be tuned based on real scenarios. A general rule for this set of hyperparameters used for \proj is that if the original CSS is large, we may want to pay attention to the reweighted message more as to alleviate the CSS. When the original shift is small, then the model may be more stable by relying on original features together with some guidance from the \proj. Other important hyperparameters are associated with the coefficient $\alpha$ for the gradient reversal layer in the adversarial training pipeline \projad. The two hyperparameters we can tune are the scale added in front of $\alpha$ and the max value that $\alpha$ can take when propagating the reverse gradients. It generally helps with the stability of adversarial training.  

\iffalse
\begin{table*}[t]
%\fontsize{6}{7}\selectfont
%\setlength\tabcolsep{1.5pt}
    \centering
    %\begin{minipage}{1.00 \linewidth}
    %\caption{Scale generalization performance on the max clique (MC) problem. Optimal solutions are generated via Gurobi9.5 with the time limit $3000$ seconds. Approximation rate larger than $1$, highlighted by $^*$, indicates the model outperforms Gurobi9.5 solver with $3000$s time budget.}
        \caption{Scale generalization performance on the MC and MVC problems. ApR is the larger the better for MC while the smaller the better for MVC. All the models are trained on RB500 training data. `Fast/Medium/Accurate' denotes GNNs (without fine-tuning) using $1/4/8$ random single node seed(s) per testing instance. `Fine-tuning' use 1-step Fine-tuning the best trial among the 8 node seed(s). `Gap' represents the averaged gap defined as $c\times($\# of nodes in the optimal solution - \# of nodes by the given method$)$ where $c=1$ for MC and $c=-1$ for MVC. `Rank' is the averaged ranks of solutions among the three methods. Optimal solutions are generated via Gurobi9.5 with the time limit $3000$ seconds. Approximation rate for MC larger than $1$, highlighted by $^*$, indicates the model outperforms Gurobi9.5 solver with $3000$s time budget. Pareto-optimal results are in bold.}
    
     \label{tab:mc_generaliztaion_scale}
     \vspace{-0.2cm}
     \centering
\resizebox{1.0\textwidth}{!}{\begin{tabular}{@{}ccc|ccc|ccc|ccc|ccc@{}}
\toprule
& \multirow{2}{*}{Dataset} & \multirow{2}{*}{Method} & \multicolumn{3}{c|}{Fast (1)} & \multicolumn{3}{c|}{Medium (4)} & \multicolumn{3}{c|}{Accurate (8)} & \multicolumn{3}{c}{Fine-tune} \\
& &  & ApR(s/g) & Gap & Rank & ApR(s/g) & Gap & Rank & ApR(s/g) & Gap & Rank & ApR(s/g) & Gap & Rank \\ \midrule
\multirow{10}{*}{MC} & \multirow{3}{*}{RB1000} &  EGN & 0.6462±0.282(0.05) & 11.48 & 2.406 & 0.8433±0.229(0.17) & 6.47 & 2.237 & 0.9099±0.205(0.33) & 4.86 & 2.025 & 0.9631±0.186(0.98) & 4.13 & 1.693 \\
 && Meta-EGN & 0.7692±0.276(0.05) & 8.57 & 1.943 & \textbf{0.9388±0.196(0.17)} & \textbf{4.61} & \textbf{1.543} & \textbf{0.9408±0.205(0.33)} & \textbf{4.97} & \textbf{1.581} & \textbf{0.9745±0.195(0.98)} & \textbf{4.01} & \textbf{1.625} \\
 & & Gurobi9.5 & \textbf{0.8851±0.197(6.11)} & \textbf{5.08} & \textbf{1.650} & 0.8851±0.197(6.18) & 5.08 & 2.218 & 0.8851±0.197(6.48) & 5.08 & 2.393 & 0.8851±0.197(7.01) & 5.08 & 2.681 \\ \cmidrule(l){2-15} 
& \multirow{3}{*}{RB2000} & EGN & 0.6793±0.290(0.10) & 12.38 & 2.408 & 0.8968±0.184(0.29) & 5.23 & 2.136 & 0.9454±0.160(0.58) & 3.81 & 2.208 & 0.9714±0.154(2.03) & 3.61 & 1.983 \\
& & Meta-EGN & 0.8077±0.114(0.10) & 8.13 & 1.991 & \textbf{0.9783±0.157(0.29)} & \textbf{3.48} & \textbf{1.591} & \textbf{0.9958±0.146(0.58)} & \textbf{1.28} & \textbf{1.466} & \textbf{1.0112±0.134(2.03)}$^*$ & \textbf{0.55} & \textbf{1.483} \\
& & Gurobi9.5 & \textbf{0.9510±0.145(24.14)} & \textbf{3.01} & \textbf{1.600} & 0.9510±0.145(24.56) & 3.01 & 2.091 & 0.9510±0.145(25.01) & 3.01 & 2.325 & 0.9510±0.145(25.66) & 3.01 & 2.533 \\ \cmidrule(l){2-15}
& \multirow{4}{*}{RB5000} & EGN & 0.9603±0.159(0.33) & 2.42 & 2.130 & 1.0203±0.139(1.02)$^*$ & -1.26 & 2.060 & 1.0272±0.140(2.50)$^*$ & -1.68 & 1.980 & 1.0475±0.188(9.66)$^*$ & -2.86 & 1.970 \\
& & Meta-EGN & \textbf{1.0288±0.138(0.33)}$^*$ & \textbf{-1.62} & \textbf{1.820} & \textbf{1.0684±0.233(1.02)}$^*$ & \textbf{-4.02} & \textbf{1.820} & \textbf{1.0727±0.234(2.50)}$^*$ & \textbf{-4.42} & \textbf{1.790} & \textbf{1.0778±0.233(9.66)}$^*$ & \textbf{-4.72} & \textbf{1.710} \\
& & Gurobi9.5 & 1.0000(201.55) & 0.00 & 2.050 & 1.0000(202.36) & 0.00 & 2.120 & 1.0000(205.64) & 0.00 & 2.230 & 1.0000(214.35) & 0.00 & 2.320 \\
& & Gurobi9.5 & 1.0000(3000) & 0.00 & - & 1.0000(3000) & 0.00 & - & 1.0000(3000) & 0.00 & - & 1.0000(3000) & 0.00 & - \\ %\bottomrule
%\end{tabular}}
     %\vspace{-0.2cm}
     %\centering
     %\fontsize{6}{7}\selectfont
%\setlength\tabcolsep{1pt}
%\resizebox{1.0\textwidth}{!}{\begin{tabular}{@{}cc|ccc|ccc|ccc|ccc@{}}
%\toprule
%\multirow{2}{*}{Dataset} & \multirow{2}{*}{Method} & \multicolumn{3}{c|}{Fast (1)} & \multicolumn{3}{c|}{Medium (4)} & \multicolumn{3}{c|}{Accurate (8)} & \multicolumn{3}{c}{Fine-tune} \\
 %&  & ApR & Gap & Rank & ApR & Gap & Rank & ApR & Gap & Rank & ApR & Gap & Rank \\ 
 \midrule
\multirow{10}{*}{MVC} & \multirow{3}{*}{RB1000} & EGN & 1.0161±0.0048(0.20) & 16.46 & 2.250 & 1.0135±0.0013(0.72) & 13.73 & 1.920 & 1.0138±0.0013(1.37) & 13.29 & 1.860 & 1.0138±0.0013(3.05) & 13.28 & 1.960 \\
&& Meta-EGN & 1.0145±0.0016(0.20) & 14.81 & 1.935 & \textbf{0.0131±0.0012(0.72)} & \textbf{13.40} & \textbf{1.700} & \textbf{1.0125±0.0012(1.37)} & \textbf{12.75} & \textbf{1.545} & \textbf{1.0124±0.0012(3.05)} & \textbf{12.69} & \textbf{1.455} \\
&& Gurobi9.5 & \textbf{1.0143±0.0018(1.92)} & \textbf{14.58} & \textbf{1.835} & 1.0143±0.0018(2.58) & 14.58 & 2.380 & 1.0143±0.0018(3.08) & 14.58 & 2.595 & 1.0143±0.0018(4.96) & 14.58 & 2.585 \\ \cmidrule(l){2-15} 
&\multirow{3}{*}{RB2000} &  EGN & 1.0114±0.0026(0.34) & 22.02 & 2.350 & 1.0096±0.0008(1.32) & 18.57 & 1.765 & 1.0094±0.0007(2.69) & 18.17 & 1.765 & 1.0093±0.0007(6.27) & 17.98 & 1.890 \\
& & Meta-EGN & \textbf{0.0103±0.0015(0.34)} & \textbf{19.94} & \textbf{1.740} & \textbf{1.0095±0.0008(1.32)} & \textbf{18.41} & \textbf{1.635} & \textbf{1.0092±0.0007(2.69)} & \textbf{17.82} & \textbf{1.510} & \textbf{1.0090±0.0006(6.27)} & \textbf{17.38} & \textbf{1.360} \\
& & Gurobi9.5 & 1.0104±0.0010(5.63) & 20.18 & 2.910 & 1.0104±0.0010(6.65) & 20.18 & 2.600 & 1.0104±0.0010(8.04) & 20.18 & 2.725 & 1.0104±0.0010(13.24) & 20.18 & 2.750 \\ \cmidrule(l){2-15} 
&\multirow{3}{*}{RB5000} & EGN & 1.0071±0.0014(1.01) & 34.19 & 2.170 & 1.0064±0.0004(3.99) & 30.83 & 1.985 & 1.0062±0.0004(7.95) & 29.87 & 1.865 & 1.0062±0.0004(18.41) & 29.68 & 1.960 \\
& & Meta-EGN & \textbf{1.0067±0.0005(1.01)} & \textbf{32.51} & \textbf{2.045} & \textbf{1.0062±0.0005(3.99)} & \textbf{29.96} & \textbf{1.600} & \textbf{1.0061±0.0004(7.95)} & \textbf{29.44} & \textbf{1.555} & \textbf{1.0060±0.0003(18.41)} & \textbf{29.15} & \textbf{1.470} \\
& & Gurobi9.5 & 1.0066±0.0006(24.60) & 31.88 & 1.785 & 1.0066±0.0006(28.72) & 31.88 & 2.415 & 1.0066±0.0006(32.16) & 31.88 & 2.580 & 1.0066±0.0006(42.62) & 31.88 & 2.570 \\ \bottomrule
\end{tabular}}
    %\end{minipage}
    \vspace{-3mm}
\end{table}
\fi




